Quantum Complexity and Holography

This thesis develops recent work on the so called Volume-Complexity and Action-Complexity conjectures. According to this family of proposals, geometric quantities can be defined in some holographic gravitational theories that can be mapped with the concept of quantum complexity for states in a dual quantum-mechanical theory. In this work, we review the original motivations for the use of quantum-information theory in the search of a theory of quantum gravity, and argue in favour of holographic complexity as a promising new tool that could play a key role in the elucidation of the properties of black holes. After this introduction, we devote some time to the study of `exotic' thermodynamical systems of diverse origin, confronting the conjectures with expectations and seeking for new behaviours of holographic complexity that could help us understand or refine the existing proposals. Next, we turn our attention to the study of holographic complexity for singular spacetimes, defining slightly modified versions of the conjecture that are well adapted to singularities and searching for universal behaviours of complexity dynamics within these setups. Finally, we finish with some speculations about the relation between holographic complexity and older characterization criteria for singularities in general relativity.

==> Chapters/Conclusions/Conclusions.tex <==
%!TEX root = ../../Thesis.tex
\chapter{Conclusions}
\label{ch:conclusions}



ehtrh

\begin{equation}
\frac{3}{4} = d
\end{equation}

\cite{Poisson}


==> Chapters/Introduction/Introduction.tex <==
%!TEX root = ../../Thesis.tex
\chapter{The strong CP problem}
\label{Ch:strong CP problem}

Let us consider the QCD Lagrangian,
\begin{equation}
\mathcal{L_{\text{QCD}}}=-\frac{1}{4} G_{\mu \nu}^{a} G^{a \mu \nu}+\theta \frac{\alpha_{s}}{8 \pi} G_{\mu \nu}^{a} \widetilde{G}^{a \mu \nu}+ \overline{Q} \left(i\slashed D -M\right)Q
\end{equation}
where $Q$ denotes a vector containing all SM quarks and $M$ is the corresponding mass matrix. 
 This Lagrangian contains two parameters that violate CP invariance, namely the $\theta$-parameter and a global phase in the quark mass matrices. But these two phases are not unrelated. 
 As we anticipated in \cref{Eq: ABJ axial anomaly,Eq:Theta bar}, by making a common axial rotation to all quarks by a phase $\beta$ both CP violating phases are shifted,\footnote{The shift on the anomalous term can be computed applying the ABJ anomaly formula with the group theory factor corresponding to a rotation of the 6 SM quarks, see \cref{Eq:Group Thepry factor anomaly}.}
\begin{equation}
 \mathcal{L}_{\cancel{CP}} = (\theta-12 \beta) \frac{\alpha_{s}}{8 \pi} G_{\mu \nu}^{a} \widetilde{G}^{a \mu \nu}- \overline{Q}  M e^{2i\beta \g_ 5}Q 
\label{Eq: axial anomaly mass term}\end{equation}
 leaving a single physical CP violating phase in the strong sector that is invarian under such field redefinitions\footnote{In the physical CP phase there is no relative factor since $\text { Arg\,(det } (M e^{2i\beta }) )=12\beta$. },
\begin{equation}
\overline{\theta} \equiv \theta_{\mathrm{QCD}}+\text { Arg\,(det } M)\,.
\end{equation}
The so called $\bar\theta$-term,
\begin{equation}
\mathcal{L_\theta}=\bar\theta \frac{\alpha_{s}}{8 \pi} G_{\mu \nu}^{a}\widetilde{G}^{a \mu \nu}
\end{equation}
  violates both parity and time reversal invariance but conserves charge conjugation  and
thus violates CP.
 As a consequence, CP violating observables such as the electric dipole moment of the neutron (nEDM) depend on the $\bar\theta$-parameter and allow to measure it. So far, experiments have not been able to measure the value of the nEDM but stringent bounds have been set, $d_n< 2.9\times 10^{-26} \text{e}\cdot \text{cm} $ \cite{Baker:2006ts}.
  There are several estimations of the theoretical value to the nEDM as a function of  $\bar\theta$ \cite{Baluni:1978rf,Crewther:1979pi,Kanaya:1981se,Schnitzer:1983pb,Cea:1984qv,Musakhanov:1984qy,Morgan:1986yy} spanning in the range $d_n=(0.1-2)\times 10^{-15} \bar\theta \,\text{e}\cdot \text{cm} $ (90\% c.l.). Using this estimations the bound on the $\bar\theta$-parameter corresponds to
\begin{equation}
|\bar\theta| <(2.9-0.2)\times 10^{-10}\,.
\end{equation}
The extremely small size of this parameter as compared to an arbitrary phase $\orderof{(\pi)}$ constitutes what we call the Strong CP. Or in other words, ``why does QCD seem not to violate CP?''. 

One may be tempted to explain the smallness of this parameter by noting that if $\bar\theta$ is set to zero, a symmetry emerges, CP, and therefore the parameter is protected by CP invariance. However this is not true since we know for a fact that CP is not a good symmetry of nature. Indeed CP violation in the weak sector is experimentally established and all observations fit in the CKM framework. Therefore the smallness of $\bar\theta$ still calls for an explanation. It should be stressed, though, that there is no theoretical inconsistency or actual experimental discrepancy with a vanishing value of $\bar\theta$. That is why some people would argue that the strong CP problem is not actually a real problem but rather a hint, a really interesting hint that can guide us in the search for a more complete theory of nature.

Although the strong CP problem can be understood in really simple terms as we have just reviewed, there are several subtleties and interesting physics behind it. Why does the $\theta$-term have physical implications if it corresponds to a total derivative?\footnote{Bardeen's identity $G_{\mu \nu}^{\alpha} \widetilde{G}^{\mu \nu \alpha}=\partial_{\mu} K^{\mu}
$.} What is an instanton and how do we know they exist? How does this relate to the missing meson problem? Why does the $\theta$-parameter describe the QCD vacuum? This chapter will be devoted to clarify these issues and gain a better understanding of the strong CP problem and the  $\bar\theta$-parameter.

\section{The missing meson problem}
Let us consider QCD with only two flavours, the up and down quarks. The fermionic Lagrangian reads,
\begin{equation}
\mathcal{L}=\overline{q} i \slashed D q- \overline{q}M_qq =\overline{q}_{L} i \slashed D q_{L}+\overline{q}_{R} i \slashed D_{R} - \left(\overline{q}_L\,M_q q_R + \hc\right)
\label{Eq: QCD two flavours}
\end{equation}
where $q_{L, R}=\left(u_{L, R}, d_{L, R}\right)^{T}$ and $M_q$ denotes the quark mass matrix,
\begin{align}\label{eq:ud_mass_matrix}
M_q=\left(
\begin{matrix}
m_u & 0\\
0 & m_d 
\end{matrix} 
\right)\,.
\end{align}
 Since the up and down quark masses are much smaller than the QCD confinement scale $m_u,\,m_d\ll \Lambda_{\text{QCD}}$, to a good approximation the second term in \cref{Eq: QCD two flavours} can be neglected. In the massless limit and at the classical level, the Lagrangian remains invariant under the following global transformation,
\begin{equation}
 \bigg(\!\!\begin{array}{c}{u_{L}} \\ {d_{L}}\end{array}\!\!\bigg) \rightarrow U_{L}\bigg(\!\!\begin{array}{c}{u_{L}} \\ {d_{L}}\end{array}\!\!\bigg), \quad\bigg(\!\!\begin{array}{c}{u_{R}} \\ {d_{R}}\end{array}\!\!\bigg) \rightarrow U_{R}\bigg(\!\!\begin{array}{c}{u_{R}} \\ {d_{R}}\end{array}\!\!\bigg)\end{equation}
 where $U_{L,R}$ are general unitary matrices. Therefore it presents a global chiral symmetry $U(2)_L\times U(2)_R=S U(2)_{L} \times S U(2)_{R} \times U(1)_{L} \times U(1)_{R}$. Their corresponding currents can be arranged into the vectorial R+L (or isospin) and baryon number currents, 
 \begin{align}
 j_V^{\mu}=\overline{q} \gamma^{\mu} q, \qquad j_V^{\mu a}=\overline{q} \gamma^{\mu} \frac{\sigma^{a}}{2} q\,,
 \end{align}
 and the axial R-L currents,
 \begin{align}
 j_A^{\mu }=\overline{q} \gamma^{\mu} \gamma^{5} q, \qquad j_A^{\mu  a}=\overline{q} \gamma^{\mu} \gamma^{5} \frac{\sigma^{a}}{2} q\,.
 \label{Eq: Currents SSB chiral}
 \end{align}
 where $\sigma^a$ are the Pauli matrices.

 As we already commented on \cref{Sec: Wigner vs Goldstone}, there are two possible fates for any symmetry of the interactions, it can be are realized \`a la Wigner-Weyl or \`a la Goldstone. Looking at the hadronic spectrum it can be easily inferred that particles form quasi degenerate multiplets of the isospin symmetry $U(2)_V=U(2)_{L+R}$, from which we conclude that the isospin symmetry is relized in the Wigner-Weyl mode. On the other hand, hadrons cannot be arranged in multiplets of the axial transformations, instead we observe light pseudoscalar particles (the three pions), that can be associated with the pseudo-Goldstone bosons of the axial currents $j_A^{\mu  a}$ in \cref{Eq: Currents SSB chiral}. Consequently, the hadronic spectrum can be understood as stemming from the  chiral symmetry breaking pattern $S U(2)_{L} \times S U(2)_{R} \times U(1)_{L} \times U(1)_{R}\longrightarrow S U(2)_{V} \times U(1)_{V}$, that is compatible with the chiral condensate taking a non-zero vacuum expectation value $\langle \bar u_L u_R +\bar d_L d_R\rangle \neq 0$.

However, the current $j_A^{\mu }$ associated to the axial symmetry $U(1)_A$ seems not to be realized in any of the two possible modes. The Wigner realization would imply the existence of a parity doubled spectrum which does not agree with experimental observations, while the Goldstone mode would imply the existence of another light pseudoscalar together with the three pions that has not been found.\footnote{The lightest pseudoscalar particle with the same quantum numbers as the axial current is the $\eta'$-meson and it has a mass of the order of that of the proton and the rest of QCD bound states $\sim\Lambda_{\text{QCD}}$, thus it cannot associated with the missing pGB.}  It was Weinberg who pointed out this issue and called it the the $U(1)_A$ problem \cite{Weinberg:1975ui} or the missing meson problem. 

The solution of this problem was found by ’t Hooft \cite{tHooft:1986ooh,tHooft:1976rip,tHooft:1976snw} who realized that the $U(1)_A$ symmetry was indeed
badly broken in QCD via the ABJ anomaly (see \cref{Sec:on broken symmetries: Anomalies}),
\begin{equation}
\partial_{\mu} j_A^{\mu}=   \frac{\alpha}{2\pi}G_{\mu \nu} \widetilde G^{\mu \nu}\,.
\end{equation}
But this is not the end of the story since the anomalous term equals a total derivative due Bardeen's identity \cite{Bardeen:1974ry},
%
\begin{equation}
G_{\mu \nu}^{\alpha} \widetilde{G}^{\mu \nu \alpha}=\partial_{\mu} K^{\mu}
\label{Eq:GGdual chern simons current}
\end{equation}
%
where $K^{\mu}=2 \epsilon^{\mu \nu \rho \sigma} \operatorname{tr}\big(A_{\nu} \partial_{\rho} A_{\sigma}-g_s\frac{2 i}{3} A_{\nu} A_{\rho} A_{\sigma}\big)$
% $K^{\mu}=\epsilon^{\mu \nu \rho \sigma} A_{\nu}^{\alpha}\big(G_{\rho \sigma}^{\alpha}-\frac{g_{s}}{3} f_{\alpha \beta \gamma} A_{\rho}^{\beta} A_{\sigma}^{\gamma}\big)$ 
is the Chern-Simons current. This facts allows to construct a new axial current whose divergence vanishes,
\begin{equation}
j'^\mu_A=j_A^{\mu}- K^\mu \,,\quad \implies \dpmu j'^\mu_A=0
\end{equation}
However, even if the anomalous term corresponds to a total derivative, there are field configurations in the QCD vacuum for which the surface integral at infinity does not vanish (see Noether's Theorem in \cref{Sec: General considerations on symmetries}). As a consecuence, the QCD anomaly explicitly breaks the axial symmetry due to instantons and the non-trivial vacuum structure of QCD, as we shall see next in more detail. After all, it became clear that the $U(1)_A$ group is not a good symmetry of QCD to begin with and therefore the spectrum does not reflect it neither manifestly nor via Goldstone modes.

With the understanding of the axial anomaly and the role of instantons, the missing meson problem was solved but another problem emerged, the strong CP problem, since it became clear that the anomalous term cannot be disregarded and deserves full consideration in light of the non-trivial QCD vacuum.


\section{QCD vacuum}

The theory of Quamtum Chrommodynamics becomes strongly coupled at low energies. Therefore the properties of the QCD vacuum can not be tacked with the usual perturbative expansions and other methods are required. In the same way that tunneling processes in Quantum Mechanics do not arise at any order of perturbation theory, QCD presents analogous phenomena to barrier penetration that require semi-classical methods. In particular, one of the best methods for computing these kind of properties of QFT is the Euclidean path integral.

Let us start by refreshing Feynman's path integral formalism in which quantum amplitudes can be expressed as sum over all possible paths interpolating from the intial state $| i\big\rangle$ to the final state $| f\big\rangle$,
\begin{equation}
\big\langle i\big|e^{-i H t / \hbar}\big| f\big\rangle= N \int[d \phi] e^{i S / \hbar}
\label{Eq:path integral feynman}
\end{equation}
In this way we can compute the probability of the initial state to time-evolve to the final state by applying the steepest descent method to compute the path integral.

Let us now consider a completely different matrix element,
\begin{equation}
\Z_{fi}(\tau)=\big\langle i\big|e^{ H \tau / \hbar}\big| f\big\rangle
%= N \int[d \phi] e^{-i S / \hbar}\,.
\label{Eq: No time evol but Euclidean}
\end{equation}
 Note that this amplitude does not correspond to the time evolution operator due to the absence of the imaginary unit $i$ and $\tau$ is just a parameter and does not correspond to the usual time\footnote{Although sometimes it can be misleading, the parameter $\tau$ is ofter dubbed imaginary time.}. This amplitude can be evaluated by inserting a basis of energy eigenstates $|n\rangle$ with corresponding energy eigenvalues $E_n$,
%  \begin{equation}
% \lim_{\tau\to\infty} \Z_{fi}(\tau)=\lim_{\tau\to\infty} \sum_n \big\langle i\big| n\big\rangle \big\langle n\big| f\big\rangle e^{ -E_n \tau / \hbar}= \big\langle i\big| \Omega\big\rangle \big\langle \Omega\big| f\big\rangle e^{ -E_0 \tau / \hbar}\,.
% \label{Eq: Capturing the vacuum}
% \end{equation}

 \begin{equation}
 \Z_{fi}(\tau)= \sum_n \big\langle i\big| n\big\rangle \big\langle n\big| f\big\rangle e^{ -E_n \tau / \hbar}\xrightarrow[]{\quad\tau\to\infty\quad} \big\langle i\big| \Omega\big\rangle \big\langle \Omega\big| f\big\rangle e^{ -E_0 \tau / \hbar}\,.
\label{Eq: Capturing the vacuum}
\end{equation}
In the limit $\tau\to\infty$, the matrix element in \cref{Eq: Capturing the vacuum} is dominated by the lowest energy eigenstate, i.e. the vacuum or ground state $\big| \Omega\big\rangle$ with energy $E_0$. As a consequence, if we are able to compute the matrix element for a given basis we can fully characterize the vacuum of the theory \cite{Coleman:1985rnk}.
 But the matrix element in \cref{Eq: No time evol but Euclidean} looks familiar, it seems analogous to that in \cref{Eq:path integral feynman}. 
Indeed if we identify $\tau=it$ we can compute $\Z_{fi}(\tau)$ with the path integral corresponding to a theory with no time but 4 spatial dimensions, i.e. the Euclidean path integral,\footnote{Under the change of variables $\tau=it$, the exponent transforms as $iS=i\int dt\Lag=i\int (-id\tau)(-\Lag_E)=-\int d\tau\Lag_E=-S_E  $}
\begin{equation}
\lim_{\tau\to\infty} \Z_{fi}(\tau)= \big\langle i\big| \Omega\big\rangle \big\langle \Omega\big| f\big\rangle e^{ -E_0 \tau / \hbar}=N \int[d \phi] e^{- S_E / \hbar}\,.
\label{Eq: Capturing the vacuumII}
\end{equation}
To sum up, we have translated the problem of characterizing the non-perturbative vacuum of a QFT in Minkowski space-time (3 spatial and one temporal dimensions), to computing the path integral for the corresponding theory with 4 spatial dimensions. If we now apply the steepest descent method to the path integral we will find that it is dominated by the stationary points of $S_E$, that is the classical solutions of finite action of the Euclidean path integral.

\subsection{Euclidean Yang-Mills theory}
Our goal now is to find all the finite action classical solutions of the Euclidean equations of motion of a Yang-Mills theory. Let us first briefly review Yang-Mills gauge theories in order to establish notational conventions that will differ from those used in the rest of the thesis. 

Yang-Mills theories are based on compact Lie groups, that have associated Lie algebras. A representation of this algebra is a set of N hermitian matrices $t^a$ satisfying the following relations,
\begin{equation}
\big[T^{a}, T^{b}\big]=i f^{a b c} T^{c}\,,\qquad \left(T^{a}\right)^{\dagger}=T^{a}\,,
\qquad \operatorname{tr} \big(T^{a} T^{b}\big)=T(R) \delta^{a b}\,,
\end{equation}
where $f^{abc}$ are the fully anti-symmetric structure constants and $T(R)$ is the Dynkin index of the representation R. The common convention for the normalization of the generators of the fundamental representation will be used, $\operatorname{tr} \big(T^{a} T^{b}\big)=\frac{1}{2} \delta^{a b}$.

\textbf{Gauge fields.} For each element of the algebra a real vector potential is introduced $A_\mu^a(x)$, i.e. the gauge fields, that can be arranged into the following matrix fields,\footnote{From now on we will refer to the generators of the fundamental representation as $T^a$ whereas the generators of a generic representation R will be $T^a(R)$.}
\begin{equation}
A_\mu (x)\equiv -ig A_\mu^a T^a\,,
\end{equation}
where  g is the gauge coupling constant. Note that this convention differs to that used in \cref{sec:The-gauge-sector} where the coupling constant is not included in the gauge potential (e.g. see Eq.~\eqref{eq:Gauge bosons}). The other difference is that throughout this section the metric that contracts the Lorentz indices is the Euclidean metric, with signature $(+,+,+,+)$ and $x_\mu=(\tau,\vec{x})$. The corresponding field strength reads,
\begin{equation}
F_{\mu \nu}=\partial_{\mu} A_{\nu}-\partial_{\nu} A_{\mu}-i\left[A_{\mu}, A_{\nu}\right]
\end{equation}
where it is implicit that $F_{\mu \nu}=F_{\mu \nu}^{a} T^{a}$.

\textbf{Gauge transformations.} In gauge theories, two field configurations are equivalent if they are related by a gauge transformation, that is a map from space\footnote{Space-time if we were considering Minkowski metric.} into elements of the Lie Group,
\begin{equation}
g(x)=e^{i\omega^a T^a}
\label{Eq:element of the gauge group}
\end{equation}
Under a gauge transformation the gauge potential and the field strength transform as follows,
\begin{equation}
A_{\mu} \longrightarrow A_{\mu}^{(g)}=g(x) A_{\mu}\, g^{-1}(x)+i g(x) \partial_{\mu} g^{-1}(x)\,,\qquad F_{\mu \nu} \longrightarrow F_{\mu \nu}^{(g)}=g(x) F_{\mu \nu}\, g^{-1}(x)\,.
\end{equation}
\subsection{Instantons}
\label{Sec:Instantons}
Now we can finally write the Euclidean action,
\begin{equation}
S_{E}=\frac{1}{4 g^{2}} \int d^{4} x F_{\mu \nu} F^{\mu \nu}\,,
\label{Eq:Euclidean action Yang Mills}
\end{equation}
that corresponds to the usual Equations of Motion (EOM) for gauge fields,
\begin{equation}
D_{\mu} F^{\mu \nu}=0\,.
\label{Eq:EOM Yang-Mills}
\end{equation}
The trivial solution to the \cref{Eq:EOM Yang-Mills} is $F_{\mu\nu}=0$, that corresponds to $A_\mu=i g(x) \partial_{\mu} g^{-1}(x)$. This solution is called ``pure gauge'' since it corresponds to gauge transformations of $A_\mu=0$ and the action density vanishes at every point of space. We are interested in finding non-trivial solutions, that is non-zero finite action solutions to \cref{Eq:EOM Yang-Mills}. Before constructing such solutions let us check if they actually exist and remind the generalization of Derrick's theorem \cite{Derrick:1964ww} to Yang-Mills theories.

\textbf{Theorem.} In Euclidean Yang-Mills theories in D spatial dimensions, the only non-singular finite-action classical solutions of the EOM are gauge transformations of $A^\mu=0$, for $D\neq4.$\\[3pt]
\textbf{Proof.} Let us assume that the field configuration $\bar A_i(x)$ is one of such finite action solutions. From it, one can construct the one-parameter family of field configurations by rescaling lengths,
\begin{align}
  A_\lambda^\mu(x) &= \lambda\,\bar A^\mu(\lambda x)\,.
\end{align}
 Due to Hamilton's principle, any solution of the classical theory has to be a stationary point of the action. As a consequence, it also has to be a stationary point among the family we have just constructed. The action scales as,
\begin{align}
S_E(\lambda) &= S_E[A_\lambda^\mu]=\lambda^{4-D}S_E[\bar A^\mu]\,.
\end{align}
For the solution to be stationary we must require that,
\begin{align}
\frac{dS_E(\lambda)}{d\lambda}\bigg|_{\lambda=1} =0\quad \implies \quad 0 =(4-D)S_E[\bar A^\mu] \,.
\label{Eq:Derricks generalization}
\end{align}
Consequently for $D\neq4$, the action needs to vanish $S_E[\bar A^\mu]=\frac{1}{4 g^{2}} \int d^{4} x F^2=0$. Since the action is the integral of a non-negative function, for the whole integral to vanish the integrand needs to be zero at every point. Therefore the only solution of the classical theory corresponds to the pure gauge $F_{\mu\nu}=0$. \hfill $\qed$
% \begin{align}
% \frac{dE(\lambda)}{d\lambda}\bigg|_{\lambda=1} =0=(4-D)E_G[\bar A^i] + (2-D) E_S[\bar \phi,\bar A^i]-DE_U[\bar \phi]
% \end{align}

Luckily, we live in 3+1 dimensions so we are interested in the 4-dimensional Euclidean Yang-Mills theory for which non-trivial solutions can exist. Let us consider the sphere at infinite radius in Euclidean space, $S^3_\infty\subset \mathbb{R}^4$. For the action to be finite we need the integrand of \cref{Eq:Euclidean action Yang Mills} to fall for large radius $r=|x|\to \infty$ faster than 
\begin{equation}
\Fmn\Fmnu\sim 1/r^{4+\epsilon}  \quad  \implies \quad \Fmn\sim 1/r^{2+\epsilon} \,,
\end{equation}
for $\epsilon>0$. One may be tempted to impose that the gauge potential needs to go as $A_\mu\sim 1/r^{1+\epsilon}$ but it would be too restrictive and the general form that $A_\mu$ can take is an arbitrary gauge transformation of the previous expression,
\begin{equation}
A_\mu\sim \orderof{\bigg(\frac{1}{r^{1+\epsilon}}\bigg)} +i g(x) \partial_{\mu} g(x)^{-1} \xrightarrow{\,\,r\to \infty\,\,}i g(x) \partial_{\mu} g^{-1}(x)\,,
\label{Eq:potential in infinity pure gauge}
\end{equation}
where $g(x)$ is a function  of the angular variables only.
We are then interested in solutions that tend to a pure gauge configuration at infinity. Those are determined by a map of the sphere at infinity to the gauge group G,
\begin{equation}
g(x):\quad S^3_\infty\,\longrightarrow \, G
%(\theta,\phi,\delta)
\end{equation}
A pertinent question now is whether any of those configurations can be gauge transformed to the trivial one. It turns out that these maps fall into disjoint classes that cannot be continuously transformed into one another, i.e. different homotopy classes. The homotopically disconnected maps from a $S^n$ sphere into some group G are classified by the group $\pi_n\left(G\right)$, which in our cases of interest is non-trivial,
\begin{equation}
% \pi_3\left(SU(2)\right)=\pi_3\left(SU(3)\right)=\mathbb{Z}\,.
\pi_3\left(SU(n)\right)=\mathbb{Z}\,, \text{  for } n\geq 2\,.
\end{equation}
This means that the connected components of the space of finite-action solutions of
 Yang-Mills $SU(n)$ theories are in one-to-one correspondence with the homotopy classes of mappings from the 3-sphere to the gauge group, that corresponds to $\pi_3\left(SU(n)\right)=\mathbb{Z}$, that is nothing but the set of integer numbers. 

The integer that allows to classify these topologically disconnected solutions is the winding number $\nu$, or Pontryagin number for the mathematically oriented, and can be computed for any such map,
\begin{equation}
\nu(g)=\frac{1}{24 \pi^{2}} \int_{\mathbf{S}^{3}} d\theta_1d\theta_2d\theta_3 \epsilon^{i j k} \operatorname{tr}\big(g^{-1} \partial_{i} g g^{-1} \partial_{j} g g^{-1} \partial_{k} g\big)\,,
\label{Eq: winding gauge}
\end{equation}
where $\theta_1,\,\theta_2,\,\theta_3$ are three angles parametrizing $S^3$.\footnote{The choice of angles is irrelevant since the Jacobian of the change of variables cancels that of the $\epsilon$-symbol.}
The winding number is a topological quantity that only depends on the boundary conditions of the field configuration, in this case on the values of the gauge potential in the sphere $S^{3}$ at infinity. It is easy to get an intuitive idea of its meaning in the case of maps of a circle into a circle,  $\pi_1(S^1)=\mathbb{Z}$, where the winding number counts the number of times the circle in field space is wrapped around the circle in ordinary space. Gauge transformations
% \footnote{Here we refer to \emph{small} gauge transformations that are those that can be smoothly deformed to the identity (they are homotopic to the identity). For a discussion on \emph{small} vs \emph{large} gauge transformations see  \cref{Sec:the theta vacuum}. }  
transform a given map $g(x)$ into another belonging to the same homotopy class, i.e. same winding number. Thus, the gauge-invariant quantity associated to finite-action solutions is not a map but its homotopy class, given by the winding number.
By making use of \cref{Eq:potential in infinity pure gauge} in \cref{Eq: winding gauge} one can express the winding number in terms of the tangential components to the 3-sphere of the gauge potential,
\begin{align}
\nu=-\frac{i}{24 \pi^{2}} \int_{\mathbf{S}^{3}} d\theta_1d\theta_2d\theta_3 \epsilon^{i j k} \operatorname{tr}\left(A_iA_jA_k\right)=
-\frac{i}{24 \pi^{2}} \int_{\mathbf{S}^{3}} d^{3} S_{\mu} \epsilon^{\mu \nu \rho \sigma} \operatorname{tr}\left(A_\nu A_\rho A_\sigma \right)\,.
\end{align}
This surface integral can be translated into an integral over the volume,
\begin{align}
 \nu=-\frac{i}{24 \pi^{2}} \int_V dx^4 \pmu \epsilon^{\mu \nu \rho \sigma} \operatorname{tr}\left(A_\nu A_\rho A_\sigma \right) = \frac{1}{16 \pi^{2}} \int_V dx^4 \pmu \epsilon^{\mu \nu \rho \sigma} \operatorname{tr}\bigg(\frac{-2 i}{3}A_\nu A_\rho A_\sigma \bigg)\,\nn\\
 =\frac{1}{32 \pi^{2}} \int_V dx^4 \pmu 2\epsilon^{\mu \nu \rho \sigma} \operatorname{tr}\bigg(A_{\nu} \partial_{\rho} A_{\sigma}-\frac{2 i}{3}A_\nu A_\rho A_\sigma \bigg)=
 \frac{1}{32 \pi^{2}} \int_V dx^4 \pmu K^\mu  \,
 \label{Eq: WInding volume anomalous term vs surface chern}
 \end{align} 
 which can be recognized to be the integral of the divergence of the Chern-Simons current $K^\mu$. Therefore applying \cref{Eq:GGdual chern simons current} we finally obtain that the winding number corresponds to the integral over the volume of the anomalous term,\footnote{Note that $\pmu K^\mu=2 \operatorname{tr}(F \widetilde{F})= F \widetilde{F}$.}
 \begin{equation}
\nu=\frac{1}{32 \pi^{2}} \int d^{4} x F \widetilde{F}\,.
\label{Eq: WInding volume anomalous term}
\end{equation}
Strikingly, by solving the classical EOM of Yang-Mills theory in Euclidean space, we found that there are non-trivial finite-action solutions, called instantons or pseudoparticles, for which the integral of the anomalous term is non-zero, and proportional to a topological charge, the winding number. This starts to indicate that there is no good reason to neglect the $G\widetilde{G}$ term in the QCD Lagrangian even though it corresponds to a total derivative, but it will become more clear in \cref{Sec:the theta vacuum} were the $\theta$-vacuum is discussed. 
% \begin{equation}
% K^{\mu}=\epsilon^{\mu \nu \rho \sigma} \operatorname{tr}\big(A_{\nu} \partial_{\rho} A_{\sigma}-g_s\frac{2 i}{3} A_{\nu} A_{\rho} A_{\sigma}\big)
% \end{equation}r



\subsubsection{The instanton action}
In order to construct instanton solutions, it is really useful to realize that these kind of solutions are stationary ponits of the action, therefore they have lower action than any other solutions in the same homotopy class (i.e. same winding number). As a consequence instantons need to saturate the \emph{Bogomol’nyi bound} \cite{Bogomolny:1975de},
 \begin{equation}
S_{E}=\frac{1}{4g^2} \int d^{4} x F_{\mu \nu} F^{\mu \nu}=\frac{1}{4g^2} \int d^{4} x\left[F \widetilde{F}+\frac{1}{2}(F-\widetilde{F})^{2}\right]=\frac{8 \pi^{2} \nu}{g^{2}}+\frac{1}{8g^2} \int d^{4} x(F-\widetilde{F})^{2}\,.
\label{Eq:bogomolnyi bound instanton}
 \end{equation}
 Since the last term of the \cref{Eq:bogomolnyi bound instanton} is possitive, the euclidean action of any field configuration with winding number $\nu$ has to be larger than the instanton solution with the same winding number, 
% \begin{equation}
% S_{E}[A] =\frac{1}{4g^2} \int d^{4} x F_{\mu \nu} F^{\mu \nu}\geq \frac{8 \pi^{2} \nu}{g^{2}}=\frac{1}{4} \int d^{4} x F \widetilde{F}=S_{E}[A_{\text{inst}}^\nu]
% \end{equation}
\begin{equation}
S_{E} =\frac{1}{4g^2} \int d^{4} x F_{\mu \nu} F^{\mu \nu}\geq \frac{8 \pi^{2} \nu}{g^{2}}
%=\frac{1}{4} \int d^{4} x F \widetilde{F}=S_{E}[A_{\text{inst}}^\nu]
\end{equation}
The inequality is saturated by the instanton solutions,
\begin{equation}
S_{E}\big|_{\nu\text{-inst}} = \frac{8 \pi^{2} \nu}{g^{2}}\,.
\end{equation}
 for which the the last term of the \cref{Eq:bogomolnyi bound instanton} needs to vanish, obtaining the self-duality equations,
\begin{equation}
F=\pm \widetilde{F}\,.
\end{equation}
Thanks to the Bogomol’nyi argument now we only need to solve the self-duality equations that are first-order differential equations instead of the full EOM,\footnote{Any  self-dual configuration solves the Yang-Mills EOM  $D_{\mu} F^{\mu \nu}=D_{\mu} \widetilde{F}^{\mu \nu}=0$ due to the Bianchi identity.} that are of second order. The anti self-dual solutions $F=- \widetilde{F}$  are called anti-instantons and have negative winding number. Once we have constructed an instanton solution it is easy to build the corresponding anti-instanton by making a parity transformation $\vec{x} \rightarrow-\vec{x} \implies F \widetilde{F} \rightarrow-F \widetilde{F} \implies \nu \rightarrow-\nu$.

\subsubsection{The BPST instanton}
We will now proceed to construct explicitly such instanton solutions with $\nu=1$ for a $SU(2)$ gauge group. We are choosing $SU(2)$ not only because it is the simplest group we can consider (for $U(1)$ every solution is trivial, $\pi_3(U(1))=0$) but also because the $SU(2)$ instantons allow us to construct instantons for any other gauge group containing a $SU(2)$ subgroup. This is a consequence of Bott's theorem \cite{Bott:1956tf} that states that any mapping from $S^3$ to a general simple Lie group $G$ can be continuously deformed into a mapping into a $SU(2)$ subgroup of $G$.

Since the relevant information of an instanton, the winding number, is solely encoded in its gauge configuration in the 3-sphere at infinity, let us start by specifying $A_\mu(|x|\to\infty)$, that needs to correspond to a pure gauge configuration. Thus this configuration at infinity is determined by a map from the $S^3$ to the gauge group. For $\nu=1$, we can define the identity map,
\begin{equation}
 g^{(1)}=\frac{\tau+i \vec{x} \cdot \vec{\sigma}}{r}
 \label{Eq: Identity map instanton}
 \end{equation} 
 As \cref{Eq:element of the gauge group} shows, an element of the gauge group $g$ is determined by the coefficients of the linear combination of the generators in the exponential, $\omega^a$. In the identity map, each point of space is mapped to the gauge group element whose coefficients determining this linear combination coincides with the normalized position vector of that point, $\omega^a=x^a=(\tau,x,y,z)$. The gauge potential at infinity is obtained by plugging the gauge group element of \cref{Eq:element of the gauge group} in \cref{Eq:potential in infinity pure gauge},
\begin{equation}
A_\mu \xrightarrow{\,\,r\to \infty\,\,}i \left(\frac{\tau+i \vec{x} \cdot \vec{\sigma}}{r}\right) \partial_{\mu} \left(\frac{\tau+i \vec{x} \cdot \vec{\sigma}}{r}\right)^{-1}\,,
\label{Eq:Instanton potential in infinity pure gauge}
\end{equation}
In order to extend the field configuration to all points in space, one can multiply \cref{Eq:Instanton potential in infinity pure gauge} by a function $f(r^2)$ that fulfills two conditions, $f(r^2)\xrightarrow{r\to 0}0$ to avoid a singularity in the origin, and $f(r^2)\xrightarrow{r\to \infty}1$ to recover the pure gauge configuration \cref{Eq:Instanton potential in infinity pure gauge} at infinity. The self-duality condition can be solved applying these conditions obtaining the  Belavin, Polyakov, Schwarz and Tyupkin (BPST) instanton solution, \cite{Belavin:1975fg}
\begin{equation}
A_\mu(x)=if(r^2)\, \left(\frac{\tau+i \vec{x} \cdot \vec{\sigma}}{r}\right) \partial_{\mu} \left(\frac{\tau+i \vec{x} \cdot \vec{\sigma}}{r}\right)^{-1}\,,\qquad f(r^2)=\frac{r^{2}}{r^{2}+\rho^{2}}
\label{Eq: The BPST instanton}
\end{equation}
that can be written in a more compact way by making use of the four dimensional Pauli matrices $\sigma^{\mu}=(\mathds{1}, i\vec{\sigma})$ as,
 \begin{equation}
A_\mu(x)=i\frac{x_\nu\sigma_{\mu\nu}}{r^{2}+\rho^{2}}\,, 
\label{Eq: The BPST instanton II}
\end{equation}
where $\sigma^{\mu \nu}=\frac{1}{2}\left(\sigma^{\mu} \overline{\sigma}^{\nu}-\sigma^{\nu} \overline{\sigma}^{\mu}\right)$ and  $\overline{\sigma}^{\mu}=(I, -i\vec{\sigma})$. 
 % $x_\mu=(\tau,\vec{x})$

However this is not the only possible solution and new configurations can be obtained by applying the symmetries of the theory. By making scale transformations, the size of the instanton $\rho$ gets modified. It is clear that we can associate the parameter $\rho$ with the size of the instanton since for $r\gg\rho$ the gauge potential approximates to pure gauge and therefore at those points $\Fmn \to0$ while for smaller values of the radius the configuration departures from pure gauge $\Fmn \neq0$ and we get most of the contribution to the action. That is why we can say that the action localized in a region with size $\rho$. In addition, one can perform a translations that would change the position of the instanton,
\begin{equation}
f(r^2)=\frac{(r-x_0)^{2}}{(r-x_0)^{2}+\rho^{2}}
\end{equation}
which adds four parameter to the family of solutions. Finally the orientation of the instanton in the group space gives 3 more parameters, that can be understood either as the three possible spatial rotations or the three constant (global) gauge transformations \cite{Jackiw:1976fs}. Summing up, the BPST instanton consists on a 8-parameter family of solutions of the Euclidean action, one for the size $\rho$, four for the position $x_0$ and three for the orientation in group space.

Finally one can build instantons with larger winding number by following the same procedure but substituting the standard map in \cref{Eq: Identity map instanton} by the following map,
\begin{equation}
 g^{(\nu)}=\left(\frac{\tau+i \vec{x} \cdot \vec{\sigma}}{r}\right)^\nu
 \label{Eq: Standard winding nu map instanton}
 \end{equation} 
which has  winding number $\nu$, as it can easily proved noting that the winding number is additive $\nu(g_1\cdot g_2)=\nu(g_1)+\nu(g_2)$.

Although we have only constructed the $SU(2)$ instantons, Bott's theorem allows to obtain instantons in any group $G\supset SU(2)$, as we already commented, by embedding $SU(2)$ instantons into $G$. Of particular interest is $G=SU(N)$, in this case one possible embedding is given by,
\begin{equation}
A_{\mu}^{S U(N)}=\left(\begin{array}{cc}{0} & {0} \\ {0} & {A_{\mu}^{S U(2)}}\end{array}\right)\,,
\end{equation}
and it can be shown \cite{Vandoren:2008xg} that by making constant gauge transformations belonging to the coset space $SU(N)/(SU(N-2)\times U(1))$ new solutions can be constructed, resulting on a family of solutions with $4N-5$ parameters. Together with the position and size already discussed it gives a total of $4N$ parameters or collective coordinates for a one instanton solution in $SU(N)$.
\subsection{Euclidean instantons as tunneling in Minkowski}
% \red{Tong (+ - - -) Why dont I call it chern simons number???} 

Once the finite-action classical solutions of Yang-Mills theories have been classified and explicitly constructed, we can go back to our original goal of understanding the QCD vaccum in Minkowski space-time. 
As we shall see in this section, instanton configurations can be interpreted as paths in Minkowski spacetime producing tunneling between classical vacua. 
Consequently, the single physical quantum vacuum corresponds to a linear superposition of the classical vacua determined by the tunneling probability \cite{Gervais:1977nv,Coleman:1977py}
. 

First let us consider the classical vacua of QCD in Minkowski space-time. The Hamiltonian density reads
\begin{equation}
\mathcal{H}=\frac{1}{2}\big(\vec{E}^{a}\big)^{2}+\frac{1}{2}\big(\vec{B}^{a}\big)^{2}\,,
\end{equation}
where $E^a_{i}=F^a_{0 i}\,,\, B^a_{i}=-\frac{1}{2} \epsilon_{i j k} F^a_{j k}$. Classical vacua have vanishing energy density and therefore $\vec{E}^{a}=\vec{B}^{a}=0\implies \Fmn=0$ at every point of space-time or, in other words, they correspond to pure gauge configurations.\footnote{It can be shown that in 3 spatial dimensions there are no time-independent non-dissipative finite-energy classical solutions of Yang-Mills, following a similar proof to that in \cref{Sec:Instantons}. Thus the only classical solution corresponds to $\Fmn=0$.} Quantum effects dramatically change this picture, though. As we have already anticipated, instantons produce tunneling between classical vacua so they will evolve in time. 

% If at a given time $t_1$ the configuration  $A_{\mu}(\vec{x}, t)$ describes a classical vacuum

% a given configuration with $\Fmn=0$ at a time $t_1$ will tunnel into a different configuration at time $t_2$. it is interesting to classify 


Let us consider the analytic continuation of the one-instanton solution in \cref{Eq: The BPST instanton} to the Minkowski space-time,  $A_{\mu}(\vec{x}, t)=A^E_{\mu}(\vec{x}, \tau=it)$ filling the volume delimited by the cylinder depicted in TAL. The winding number can still be defined and computed even though we are in Minkowski because it is a topological quantity that does not depend on the metric,
 \begin{equation}
\nu=\frac{1}{32 \pi^{2}} \int d^{4} x F \widetilde{F}=
-\frac{i}{24 \pi^{2}} \int_{\text{I+II+III}} d^{3} S_{\mu} \epsilon^{\mu \nu \rho \sigma} \operatorname{tr}\left(A_\nu A_\rho A_\sigma \right)\,.
\label{Eq:winding minkowski instanton}
\end{equation}
 Since the instanton has finite action, the field configuration is pure gauge in all the surfaces at infinity. In particular, at initial time $t_1\to-\infty$ the configuration $A_{\mu}(\vec{x}, t_1)$ describes a classical vacuum,
\begin{equation}
A_{\mu}(\vec{x}, t_1)=i g(\vec{x}, t_1) \partial_{\mu} g^{-1}(\vec{x}, t_1)\,,
\end{equation}
and analogously, for $t_2\to\infty$ the configuration describes another classical vacuum,
\begin{equation}
A_{\mu}(\vec{x}, t_2)=i g(\vec{x}, t_2) \partial_{\mu} g^{-1}(\vec{x}, t_2)\,.
\end{equation}
Finally the remaining boundary is also pure gauge,
\begin{equation}
A_{\mu}(\vec{x}, t)\xrightarrow{\,|\vec{x}|\to\infty\,}i g(\vec{x}, t) \partial_{\mu} g^{-1}(\vec{x}, t)\,.
\label{Eq:pure gauge boundary III}
\end{equation}
In order simplify our arguments we can choose the gauge,
\begin{equation}
A_{0}(\vec{x}, t)=0\,,\qquad A_{\mu}\left(\vec{x}, t_{1}\right)=0
\label{Eq gauge fixing}
\end{equation}
that corresponds to the temporal gauge (in every point of space-time) and to setting the gauge potential to zero in the initial vacuum with the residual space-dependent gauge freedom, $g(\vec{x}, t_1)=1$. \\
With this gauge fixing, the field configuration in the boundary III vanishes. Combining \cref{Eq:pure gauge boundary III,Eq gauge fixing} we conclude that $g(|\vec{x}|\to\infty,t)$ does not depend on time  and because on the surface I the gauge potential vanishes, $A_{\mu}\left(\vec{x}, t_{1}\right)=0$, it must vanish for all $t$, therefore,
\begin{equation}
A_{\mu}(\vec{x}, t)\xrightarrow{\,|\vec{x}|\to\infty\,}0\,.
\end{equation}
This has an interesting consequence in terms of classifying classical vacua in Minkowski. For every spatial slice $t=\text{cte}$, in the limit $|\vect{x}|\to \infty$ the gauge potential vanishes. Thus this hypersurfaces can be compactified into 3-spheres in which the north pole is associated with all the points at $|\vect{x}|\to \infty$. Hence the initial $t_1$ and final $t_2$ slices that correspond to classical vacua can be classified by the maps from a 3-sphere into the gauge group, i.e. the winding number.
\begin{equation}
n(t)=
-\frac{i}{24 \pi^{2}} \int_{{S_t}} d^{3} x^3 \epsilon^{0 ijk} \operatorname{tr}\left(A_i A_j A_k \right)
\label{Eq: winding non integer}
\end{equation}
Now we can relate the winding number of the instanton with the winding number of the initial and final classical vacua, from \cref{Eq:winding minkowski instanton},
 \begin{equation}
\nu=-\frac{i}{24 \pi^{2}} \int_{\text{I+II+III}} d^{3} S_{\mu} \epsilon^{\mu \nu \rho \sigma} \operatorname{tr}\left(A_\nu A_\rho A_\sigma \right)=n_2-n_1\,.
\label{Eq:winding n1-n2}
\end{equation}
since the integral on the boundary III vanishes.

Several comments are pertinent. The fact that the winding number defined in \cref{Eq: winding non integer} is computed by integrating over an open surface in Minkowski space-time makes it qualitatively different from the winding number of instantons in Euclidean space. On the one hand, time evolution can smoothly deform a configuration with certain winding number to another one with different winding. 
Indeed, the winding number can be computed for any spatial slice $t=\text{cte}$ by making use of \cref{Eq: winding non integer} and from the initial to final configurations $n(t)$ continuously interpolates between $n_1$ and $n_2$, taking non-integer values in between where the field configurations are not pure gauge. On the other hand, so-called large gauge transformations can change the winding number that classifies the classical vacua in Minkowski space-time.\footnote{This gauge transformation corresponds to the space-dependent gauge fixing we used to fix the potential in $t=t_1$ in \cref{Eq gauge fixing}. They are called \emph{large} because they do not approach the identity at infinity.} 
However if one performs one of such gauge transformations and increases the winding number at time $t_1$ by m units, $n_1\to n_1+m$, then the winding number at time $t_2$ increases by exactly the same amount $n_2\to n_2+m$, rendering the total winding number that corresponds to that of the Euclidean instanton gauge invariant.\\
This can be easily understood by noticing that while the anomalous term $F\widetilde F$ is gauge invariant, the Chern-Simons current $K^\mu$ is not. If we are computing the winding number integrating the Chern-Simons current over a closed surface, it can be translated into an integral over the volume of the anomalous term and therefore the result will be gauge invariant, see \cref{Eq: WInding volume anomalous term vs surface chern}. If the surface over which we integrate is open instead, it cannot be written as a function of gauge invariant operators and the winding number will be shifted under large gauge transformations. 

As we already commented, there are no classical paths that connect two vacua with different winding numbers since the only classical solution corresponds to pure gauge in all points of space-time. 
 Therefore, this path determined by the instanton solution necessarily involves non-vanishing $\Fmn$ and therefore non-vanishing energy density at some intermediate times (otherwise the total winding number vanishes).
 For this reason these transitions look like tunneling processes between two classical vacua since they are classically forbidden but quantum mechanically allowed  via barrier penetration.
 Indeed it can be shown \cite{Bitar:1977wy} that the instanton solution gives rise to the maximal tunneling amplitude in Minkowski space. This probability is related to the Euclidean action of the corresponding instanton, see \cref{Eq: Capturing the vacuum},
\begin{equation}
P\propto e^{-S_E/\hbar}=e^{-\frac{8\pi^2}{g^2\hbar}|\nu|}\,,
\end{equation}
where $\nu$ is the difference between the winding numbers of the two classical vacua that are connected by this tunneling. We obtain the characteristic dependence on the coupling constant of non-perturbative effects $\propto e^{-1/g^2}$ that does not arise
at any level in perturbation theory.
 In fact, instanton techniques can be used to compute barrier penetration amplitudes generically in Quantum Mechanics problems obtaining the same semiclassical result that is usually computed using the WKB approximation.


We have showed that an instanton configuration with a given size, position, direction and winding number $\nu$ produces tunneling between two classical vacua whose winding differ by the instanton winding number $\nu=n_2-n_1$. Nevertheless, if we wish to compute the full probability for a transition from a two classical vacua $|m\rangle$ to $|n\rangle$ one needs to integrate over all possible instanton configurations compatible with that difference in winding number,
\begin{equation}
\big\langle n\big|e^{- H \tau/ \hbar}\big| m\big\rangle=\int[d A]_{(n-m)} e^{- S_E/ \hbar}\,.
\label{Eq: m-n instanton}
\end{equation}
In order to evaluate this integral one can use the dilute instanton gas approximation (DIGA). By assuming that all the instanton configurations contributing to the integral are widely separated as compared to their size $\rho$, the matrix element reads,
\begin{equation}
\Z_{1,0}(\tau)=\langle 1|e^{-H \tau/ \hbar}| 0\rangle=C V \tau \int \frac{d \rho}{\rho^{5}}\left(\frac{8 \pi^{2}}{{g}^{2}(1 / \rho)\hbar}\right)^{2 N} e^{-\frac{8 \pi^{2}}{{g}^{2}(1 / \rho )\hbar}} \,.
\label{Eq: Dilute instanton gas approx}
\end{equation}
where $C$ is a constant that depends on the number of colors $N$ for a given $SU(N)$ theory that arises after performing the integration over all the posible the directions is group space of the instantons and $V\tau$ is the Euclidean volume that is obtained after integrating over the instanton positions. It must be noted that this approximation is not valid in for small scales (large instanton sizes). Indeed the integral in \cref{Eq: Dilute instanton gas approx} diverges generating what `t Hooft called an \emph{infrared embarrassment}. After all this divergence should not be a surprise since the QCD coupling constant becomes large at low energies where we enter a strongly coupled regime in which the semi-classical approximation that has been assumed does not apply. Although for confining theories the DIGA cannot be applied and we are not able to compute the full integral in \cref{Eq: m-n instanton}, the rest of the discussion holds and it is enough in order to characterize the vacuum of the theory.

\subsection{\texorpdfstring{$\theta$} --vacuum}
\label{Sec:the theta vacuum}
 The classical vacua labelled by the winding number $|n\rangle$ in Minkowski space have all the same (vanishing) energy. However, similarly to quantum mechanics, the degeneracy between different classical vacua is lifted if there exists tunnelling between them.  In order to construct the linear combination of the different states $|n\rangle$ that corresponds to the true quantum vacuum, we are going to impose that it has to be gauge invariant. Large gauge transformations such as,
 \begin{equation}
 T_{1}(\vec{x},t)=\frac{i \vec{x} \cdot \vec{\sigma}}{\left(\vec{x}^2+a^2\right)^{1/2}}
 \label{Eq: LGT instanton}
 \end{equation}
 increase the winding number of a classical state by one unit, $ T_1|n\rangle=|n+1\rangle$. However, the physical quantum vacuum needs to be invariant under such transformation and in a Hilbert space that amounts to obtaining the same state modulo a phase, $T_1|\text{vac}\rangle=e^{i \theta}|\text{vac}\rangle$. If the quantum vacuum is expressed as a linear combination of the classical states, by imposing gauge invariance one can obtain a relation among the coefficients,
\begin{align}
|\text{vac}\rangle=\sum_{n=-\infty}^{\infty} a_n|n\rangle\,\implies T_1|\text{vac}\rangle=\sum_{n=-\infty}^{\infty} a_n|n+1\rangle= e^{i \theta}|\text{vac}\rangle\\
|\text{vac}\rangle=  e^{-i \theta}\sum_{n=-\infty}^{\infty} a_n|n+1\rangle=  \sum_{n=-\infty}^{\infty} e^{-i \theta} a_{n-1}|n\rangle=\sum_{n=-\infty}^{\infty} a_n|n\rangle
\end{align}
Then the coefficients need to follow the recursive relation $a_{n+1}=e^{-i \theta}a_n$. By choosing $a_0=1$, that only corresponds to a choice of normalization, we unambiguously find the true vacuum \cite{Jackiw:1976pf}, that can be labelled by the phase $|\text{vac}\rangle\equiv |\theta\rangle$,
\begin{equation}
|\theta\rangle=\sum_{n=-\infty}^{\infty} e^{-i n \theta}|n\rangle\,.
\end{equation}
After all this analysis we have arrived to the conclusion that the vacuum of Yang-Mills is characterized by a phase $\theta$ that determines the linear superposition of the classical vacua in the true quantum ground state. But, do states with different values of $\theta$ correspond to different states in the same theory? 
\begin{equation}
\begin{aligned}
\big\langle\theta^{\prime}\big|e^{-i H t/ \hbar}\big| \theta\big\rangle &=\sum_{m, n} e^{i m \theta^{\prime}} e^{-i n \theta}\big\langle m\big|e^{-i H t/ \hbar}\big| n\big\rangle \\ 
&=\sum_{m, n} e^{i m(\theta^{\prime}-\theta)} e^{i(m-n) \theta}\big\langle m\big|e^{-i H t/ \hbar}\big| n\big\rangle \\
&=\sum_{m, k} e^{i m(\theta^{\prime}-\theta)} e^{i k \theta}\big\langle k\big|e^{-i H t/ \hbar}\big| 0\big\rangle = 2 \pi \delta\big(\theta-\theta^{\prime}\big) \sum_{k} e^{i k \theta}\big\langle k\big|e^{-i H t/ \hbar}\big| 0\big\rangle \end{aligned}
\label{Eq:theta theta'}
\end{equation}
Time evolution does not connect states with different $\theta$'s. In fact, it can be shown that the matrix element of any string of local observables $\mathcal{O}_1\ldots\mathcal{O}_k$ vanishes for $\theta'\neq\theta$, $\big\langle\theta^{\prime}\big|\mathcal{O}_1\ldots\mathcal{O}_k\big| \theta\big\rangle\propto\delta(\theta-\theta')$. This implies that different values of $\theta$ do not label states in a given theory but correspond to different theories. But, do they give different physics?
The answer is yes. The energy density of the vacuum depends on $\theta$ as it can be shown by computing the matrix element in \cref{Eq: Capturing the vacuum} for the vacuum $\big| \theta\big\rangle $ and making use of \cref{Eq:theta theta'},
\begin{equation}
\lim_{\tau\to\infty} \Z_{\theta\theta}(\tau)= \big\langle \theta\big| \theta\big\rangle  e^{ -E_0 \tau / \hbar}=e^{ -E_0 \tau / \hbar}=N \int_\theta[d A] e^{- S_E / \hbar}= \sum_{n} N \int[d A]_ n  e^{i n \theta} e^{- S_E / \hbar}\,.
\label{Eq: theta vacuum energy}
\end{equation}
Approximating again the integral in the DIGA one obtains,
\begin{equation}
e^{ -E_0 \tau / \hbar}= e^{2V\tau K \cos \theta e^{-S_0/\hbar}} \implies  \frac{E(\theta)}{V}= \text{cte}-2K \cos \theta e^{-S_0/\hbar}
\end{equation}
Therefore theories with different values of $\theta$ have different vacuum energy. Although we have used the DIGA to obtain this result, the fact that the energy density of the vacuum is $\theta$-dependent holds in any case. In fact it can be shown in all generality that the minimum energy density of the vacuum corresponds to $\theta=0$ and for any $\theta\neq 0$ the energy density is larger \cite{Vafa:1983tf}. As a consequence the value of $\theta$ of a given theory has physical impact.

We are now ready to make the connection of the $\theta$-vacuum with the $\theta$-term appearing in the Lagrangian. The vacuum expectation value of any operator $\mathcal{O}$ can be expressed as,
\begin{equation}
\begin{aligned}
\langle\theta|\mathcal{O}| \theta\rangle &=
\sum_{m, n} e^{i \theta(m-n)}\langle m|\mathcal{O}| n\rangle=
\sum_{k} e^{i \theta k}\langle k|\mathcal{O}| 0\rangle=
\sum_{k} e^{i \theta \int d^{4} x \frac{1}{32 \pi^{2}} G \tilde{G}}\langle k|\mathcal{O}| 0\rangle \\
 &=\frac{1}{\mathcal{Z}}\sum_{k} \int \left[d A\right]_k \mathcal{O}\, e^{i \int d^{4} x \left(\mathcal{L}+\frac{\theta}{32 \pi^{2}} G \tilde{G}\right)}=\frac{1}{\mathcal{Z}}\int\left[ d A\right] \mathcal{O}\,e^{i \int d^{4} x \left(\mathcal{L}+\frac{\theta}{32 \pi^2} G \tilde{G}\right)} \end{aligned}
 \label{Eq: Theta vacuum enters the Lagrangian}
\end{equation}
By using the definition of the winding number in terms of the volume integral of the anomalous term, see \cref{Eq: WInding volume anomalous term} we have found that the result of any observable in a particular vacuum $|\theta\rangle$ amounts to adding to the Lagrangian of the theory the anomalous term
\begin{equation}
\Lag_\theta = \frac{\theta}{32 \pi^2} G_{\mu \nu}^{a}\widetilde{G}^{a \mu \nu}\,.
\label{Eq: theta term end of instantons}
\end{equation}

Sumarizing, by studying the Euclidean Yang-Mills theory we found that the structure of the QCD vacuum cannot be described perturbatively. There exist an infinite number of classically degenerate
vacuum states whose coherent superposition labeled by $\theta$ defines the true QCD vacuum.  The properties of this vacuum can be studied in the semiclassical approximation by constructing the classical solutions of the Euclidean theory, that describe tunneling paths between the classical vacua in Minkowski space. Then, it has been shown that the impact on physical observables of a given $\theta$-vacuum can be encoded in the Lagrangian by introducing the corresponding $\theta$-term, see \cref{Eq: theta term end of instantons,Eq: Theta vacuum enters the Lagrangian}. As a consequence, QCD interactions are not described by a single dimensionless parameter, the coupling constant $g$, but by two parameters $g$ and $\theta$. 

Furthermore, instantons allow to solve the missing meson problem which provides experimental evidence for the explicit breaking of the $U(1)_A$ symmetry. Therefore instantons do have physical consequences and it becomes clear that the fact that the QCD vacuum is CP-invariant remains to be a puzzle calling for an explanation,a solution to the strong CP problem.
% us with the strong CP problem: why do strong interactions seem to conserve CP?

\subsection*{Adding fermions}

So far we have constructed the instantons and the $\theta$-vacuum for a pure Yang-Mills theory but since we are interested in studying QCD, fermions need to be incorporated. One of the immediate consequences of introducing fermions is that it becomes clear why the different classical topological vacua are physically distinguishable: they posses different axial charge. As we introduced in \cref{Sec:on broken symmetries: Anomalies}, the quark axial current is anomalous,
\begin{equation}
\partial_{\mu} j_A^{\mu}=   \frac{\alpha}{2\pi}G_{\mu \nu} \widetilde G^{\mu \nu}\,,
\end{equation}
and after integrating over a volume, the difference in axial charge is obtained,
\begin{equation}
\Delta Q_{A}=Q_{A}(t=+\infty)-Q_{A}(t=-\infty)=\int d^{4} x \partial_{\mu} j_{\mu}^{A}=2\,\nu\,.
\end{equation}
Therefore instantons with winding $\nu=1$ generate tunneling events in which the axial charge of the
vacuum changes by two units, therefore they generate fermionic interactions containing one quark and one anti-quark for each flavour. This can also be seen by integrating over the quark fields  in the path integral. In the semiclassical approximation the fermionic integration gives rise to the determinant of the Dirac operator in an instanton classical background $A_\mu$,
\begin{equation}
\int \big[d\psi\big] \big[d\bar\psi\big] e^{\int d^4x \bar\psi(i\slashed\partial -m-\slashed A)\psi}= \text{Det}(i\slashed\partial -m-\slashed A)\,.
\end{equation}
If the limit $m\to0$, it was shown by `t Hooft that the fermionic zero modes of the Dirac operator make the vacuum to vacuum amplitude vanish \cite{Shifman:1979uw,tHooft:1976snw,Callan:1977gz}. Instead, as we have anticipated studying the chiral charge, the tunneling amplitude is non-zero in the presence of external quarks. In this case, the zero modes of the determinant cancel with the fermionic propagators, resulting in a non-vanishing amplitude for the fermionic interaction. This corresponds to the so-called `t Hooft determinental interaction.

In the fermions are massive instead, the external legs of this determinental interaction can be closed with the mass terms, generating a non-zero vacuum to vacuum amplitude. \cite{tHooft:1976snw,Callan:1977gz,Andrei:1978xg,Baulieu:1978uu}
In the Dilute Instanton Gas Approximation where the determinant factorizes to the product of the determinants for each instanton background, this amounts to multiply the pure Yang-Mills result by a factor of $(\rho m_f)$ for each Weyl fermion\footnote{This factor $(m_f\rho )$ holds for  small instanton sizes $\rho\ll 1/m$. For large instantons $\rho\gg 1/m$ the fermions completely decouple and have no impact on the vacuum to vacuum amplitude.} 

\begin{equation}
\mathcal{Z}= C_{inst}(N_f, N_c)\int \frac{d \rho}{\rho^{5}} \prod_ f (m_f\rho)\left(\frac{8 \pi^2}{g^2(\nicefrac{1}{\rho})}\right)^{2 N_{c}} e^{-\frac{8 \pi^2}{g^2(\nicefrac{1}{\rho})}}\,,
\end{equation}
where the coefficient $C_{inst}$ for $N_f$ Weyl fermions in a $SU(N_c)$ Yang-Mills theory reads,
\begin{equation}
C_{i n s t}\left(N_{f}, N_{c}\right)=\frac{4 \cdot 2^{-2 N_{c}} e^{c_{1 / 2}\left(-2 N_{c}+2 N_{f}\right)}}{\pi^{2}\left(N_{c}-2\right) !\left(N_{c}-1\right) !} e^{-c_{1}+4 c_{1 / 2}}\,.
\label{Eq: Cinst with fermions}
\end{equation}
where the function $c(x)$ is defined in Ref.~\cite{tHooft:1976snw} such that $c(\nicefrac{1}{2}) = 0.145873$ and $c(1) = 0.443307$.




\subsection{Instantons in spontaneously broken theories: constrained instantons}
\label{Sec: constrained instantons}
Before reviewing possible solutions to the Strong CP problem let us first comment on instanton solutions in spontaneously broken gauge theories. This will be of special relevance in \cref{Chap:CUDA} where small-size instantons of this type will raise the axion mass.

At first sight it seems we arrive to a dead end since \emph{exact} instanton solutions do not exist in spontaneously broken theories. 

% In order to show it let us consider the generalization of Derrick's theorem in TAL ncluding a scalar field that takes a vacuum expectation value different from zero. 
\textbf{Theorem.} In spontaneously broken Euclidean Yang-Mills theories in 4 dimensions with the Lagrangian
\begin{equation}
\mathcal{L}= -\frac{1}{4g^2}F_{\mu\nu}^aF^{\mu\nu}_a + (D_\mu \phi)^\dagger D^\mu \phi- U(\phi) \,,
\end{equation}
 where the minimum of $U(\phi)$ corresponds to a non-vanishing value of the scalar field, $\langle\phi\rangle=v\neq 0$, the only non-singular finite-action classical solutions of the EOM are gauge transformations of $A^\mu_a=0, \phi=v$.\\[4pt]
\textbf{Proof.} The action of this theory reads
\begin{equation}
S_E[\phi,A_\mu]=S_G[A_\mu]+S_S[\phi,A_\mu]+S_U[\phi]
\end{equation}
where the three terms are non-negative and correspond to
\begin{align}
S_G[A_\mu]     &= \frac{1}{4 g^2}\int d^Dx\,F_{\mu\nu}^aF^{\mu\nu}_ a\,, \\
S_S[\phi,A_\mu]&= \int d^Dx\,(D_\mu \phi)^\dagger D^\mu \phi\,, \\
S_U[\phi]      &= \int d^Dx U(\phi)\,. \, 
\end{align}  
Analogously to \cref{Eq:Derricks generalization}, let us consider the one-parameter family of field configurations obtained by rescaling lengths in a given solution with finite action $ \{\bar A^\mu(x),\,\bar \phi(x)\}$,
\begin{align}
   A_\lambda^\mu(x) &= \lambda\,\bar A^\mu(\lambda x)\,,& \phi_\lambda(x) = \bar \phi(\lambda x)&\qquad\,
\end{align}
 whose action reads
\begin{align}
S_E(\lambda) &= S_G[A_\lambda^\mu]+S_S[\phi_\lambda,A_\lambda^\mu]+S_U[\phi_\lambda] \nonumber \\
           &=\lambda^{4-D}S_G[\bar A^\mu] + \lambda^{2-D} S_S[\bar \phi,\bar A^\mu]+ \lambda^{-D}S_U[\bar \phi]\,.
\end{align}
For the solution $\bar A_i(x)$ to be a stationary point of the action,
\begin{align}
\frac{dS_E(\lambda)}{d\lambda}\bigg|_{\lambda=1} =0\quad \implies \quad 0 =(4-D)S_G[\bar A^\mu] + (2-D) S_S[\bar \phi,\bar A^\mu]-DS_U[\bar \phi]\,.
\label{Eq:SSB instantons hamilton pple}
\end{align}
Thus for $D=4$ spatial dimensions the condition reads,
\begin{align}
 0 = -2 S_S[\bar \phi,\bar A^\mu]-4 S_U[\bar \phi]\,
\label{Eq:Derricks generalization scalar hamilton D=4}
\end{align}
Since both terms are positive both need to be zero independently, 
\begin{align}
S_S[\phi,A_\mu]&= \int d^Dx\,(D_\mu \phi)^\dagger D^\mu \phi\,, \\
S_U[\phi]      &= \int d^Dx U(\phi) \, .
\end{align}
In both cases the integrand is positive so it has to identically vanish in every point in order for the full integral to vanish,
\begin{align}
(D_\mu \phi)^\dagger D_\mu \phi&=0 \quad \forall x \label{Eq:phi}\\ 
 U(\phi) &=0 \quad \forall x 
\end{align}
Therefore the action density of the scalar field vanishes everywhere. However, \cref{Eq:Derricks generalization scalar hamilton D=4} allows for the gauge fields to have finite non-zero action. But now we will show that Eq.~\eqref{Eq:phi} implies that the gauge potential configuration corresponds to a pure gauge in every point of space and therefore all the solutions of this kind are trivial,
\begin{equation}
|D_\mu \phi|^2=0 \implies D_\mu \phi=\left(\partial_\mu +i A_\mu\right)\phi=0 \implies A_\mu\phi =i \partial_\mu\phi\,.
\label{Eq:scalar condition SSB}
\end{equation}
For the potential $U(\phi)$ to be zero, the scalar field has to be at the minimum in every point of space. Let us us consider one of such zeros of $U(\phi)$, $\phi=v$. Since $U$ is gauge invariant, any gauge transformation of it, $\phi^{(g)}=g\,v$, will also be a zero of the potential. Let us assume that all zeros of the potential are of the kind $g\,v$, excluding any accidental degeneracy or extra global internal symmetry of the Lagrangian. Then the gauge potential reads,
\begin{equation}
A_\mu= i \phi^{-1}\partial_\mu \phi=i g^{-1} v^{-1}\partial_\mu g v=i g^{-1}\partial_\mu g
\end{equation}
that corresponds to a pure gauge configuration in all points of space time and thus with vanishing action, $S_G[A_\lambda^\mu]=0$. Thus all three terms contributing to the action vanish, and we can conclude that there are no exact classical solutions with non-zero but finite action in spontaneously broken gauge theories in Euclidean space.  \hfill $\qed$

Crucially, in order to be able to infer something about the gauge potential configuration via the condition on Eq.~\eqref{Eq:scalar condition SSB}, we need the theory to be spontaneously broken, that is the scalar needs to develop a non-zero vev. Otherwise if $\langle \phi \rangle=0$, the condition in Eq.~\eqref{Eq:scalar condition SSB} is automatically satisfied and the usual instantons of Yang-Mills theory are also solutions of the theory with scalars that do not develop a vev. 

\subsection*{Constrained instantons}
Even if there are not \emph{exact} instanton solutions in spontaneously broken theories, one can construct approximate solutions for instanton sizes smaller than one over breaking scale $g \rho v\ll 1$. This is what we call constrained instantons. There are two ways of constructing them, the most rigorous approach was introduced by Affleck in Ref.~\cite{Affleck:1980mp} and consists on introducing a constraint as a Lagrange multiplier which fixes the instanton size $\rho$ for its exact solution, and then integrate over this constraint. Alternatively, one can take the approach by `t Hooft in Ref.~\cite{tHooft:1976snw} and  solve the approximate EOM of the fields for $ \rho \ll 1/(gv)$.  This approximation consists on neglecting the current induced by the non-vanishing scalar field $\phi$ in the EOM for the gauge fields,
\begin{align}
 \begin{array}{c}{D_{\mu} F_{\mu \nu}=0}\,, \\ 
 {D_{\mu} D_{\mu} \phi-U^{\prime}(\phi)=0}\,.
 \end{array}
 \end{align} 
which are solved with the boundary conditions that ensure the finiteness of the action,
\begin{align}
\qquad\quad A_{\mu}(x) &\rightarrow i g(x) \partial_{\mu} g^{-1}(x) &\text { for }r \rightarrow \infty &\quad\\ 
\phi(x) &\rightarrow g(x) v \quad &\text { for }r \rightarrow \infty&\qquad\quad
\end{align}
In other words, the approximation amounts to considering the instanton solution of pure Yang-Mills theory for small sizes, and then solving the EOM for the
scalar in this background. As a result the action contains the usual Yang-Mills instanton term plus an extra contribution from the scalar \cite{Espinosa:1989qn,Affleck:1980mp,Csaki:1998vv,Vandoren:2008xg}, yielding,
\begin{equation}
S_E= \frac{8 \pi^{2} }{g^{2}}+ 2\pi^2\rho^2 v^2\,.
\end{equation}

Although they are approximate solutions, constrained instantons can have im
mportant effects and, unlike usual instantons, they can be tackled quantitatively in a reliable way using the DIGA. The breaking scale $v$ provides a natural cut-off for the instanton size, that solves the \emph{infrared embarrassment} of the Dilute Instanton Gas Approximation of confining Yang-Mills theories. In this case the one-instanton contribution to the vacuum functional in the DIGA reads,
\begin{equation}
\mathcal{Z}= C_{inst}(N_f,N_c)\int \frac{d \rho}{\rho^{5}}\left(\frac{8 \pi^2}{g^2(\nicefrac{1}{\rho})}\right)^{2 N_{c}} e^{-\frac{8 \pi^2}{g^2(\nicefrac{1}{\rho})}-2\pi^2\rho^2 v^2}\,,
\end{equation}
where $C_{inst}$ is defined in \cref{Eq: Cinst with fermions}. The extra contribution of the scalar action to the path integral $e^{-2\pi^2\rho^2 v^2}$ exponentially suppresses large instanton sizes and makes the whole integral convergent. This type of instantons have been considered in the context of B+L violation in the Electroweak sector \cite{tHooft:1976snw,tHooft:1976rip,Shifman:1979uw,Ringwald:1989ee,Espinosa:1989qn}.

%%%%%%%%%%
%%% SOLUTIONS TO THE STRONG CP
%%%%%%%%

\section{Solutions to the strong CP problem}
\subsection*{Running of \texorpdfstring{$\bar{\theta}$} --parameter}
% \subsection{Running of \texorpdfstring{$\theta$}}
For certain solutions to the strong CP problem, it is important to take into account the running of $\theta$.
Although the $\theta$-parameter breaks CP invariance, it is not a technically natural parameter in the `t Hooft sense due to the fact that CP is already broken within the electroweak sector of the SM. 
Thus $\theta$ is not protected by a symmetry and indeed receives radiative corrections that depend on  the complex phase of the CKM matrix, $\delta_{CKM}$. 
In terms of the viability of some solutions to the Strong CP problem that set $\bar\theta=0$ at some high scale $\Lambda$, it is important to quantify these contributions. This issue was addressed by Ellis and Gaillard in Ref.~\cite{Ellis:1978hq} who found that the infinite renormalization of $\theta$ due to $\delta_{CKM}$ vanishes until 7-loops. As a consequence, even if the ``relaxation'' scale $\Lambda$ at which  $\bar\theta$ is set to zero were to be the Planck scale, this contribution is so suppressed, $\Delta \theta\sim 10^{-16}$, that can be dafely neglected as compared with the current and foreseeable experimental precision in the nEDM.

\subsection{Nelson-Barr mechanism}
One possible solution to the strong CP problem is that of spontaneously broken CP models via the Nelson-Barr mechanism \cite{Nelson:1983zb,Barr:1984qx,Barr:1984fh}
. If CP were to be an exact symmetry of the interactions, the $\theta$-term would be absent in the Lagrangian. However CP violation in the weak sector needs to be accounted for and within these models it arises through a scalar singlet that develops a complex vev, breaking spontaneously the CP symmetry. The Yukawa and mass terms are constructed in such a way that at tree level this complex vev only induces a non-zero phase in the CKM while leaving a vanishing $\theta$.

One of the simplest realizations of this mechanism \cite{Bento:1991ez}
 introduces down-type vector-like quarks $q_{L,R}$ and several complex scalar singlets $\eta_i$ with the following mass and Yukawa couplings,
\begin{equation}
\mathcal{L}\supset-\mu \,\overline{q}_L q_R-a \,\eta \overline{q}_L D_{R} -y H \overline{Q}_{L} {D}_{R}\,,
\label{Eq: Nelson Barr Lagrangian}
\end{equation}
where the flavour indices have been omitted. Note that since CP is an exact symmetry at this level the coulings $\mu,\,a\,$ and $y$ are real. At some energy scale the scalars $\eta$ develop complex vevs and break spontaneously CP invariance. After EWSB the Lagrangian in \cref{Eq: Nelson Barr Lagrangian} gives rise to the mass matrix
\begin{equation}
{M}=\left(\begin{array}{cc}{\mu} & {B} \\ {0} & {m_{d}}\end{array}\right) \,,
\end{equation}
where $m_{d} \equiv y v$ is the $3\times3$ down-type quark mass matrix and $B=a \langle\eta\rangle$. Notice that since the only complex phases in this mass matrix appear within the submatrix $B$  (both $m_d$ and $\mu$ are real) automatically  $\text { Arg\,(det } M)=0$ and at tree level there are no contributions to the $\theta$-term. On the other hand, the exotic quark gets a large mass since $\mu,a \langle\eta\rangle\gg v$ and when it is integrated out of the spectrum it introduces a complex phase in the mass matrix of the SM, giving rise to a non-zero $\delta_{CP}$ in the CKM matrix.

Nevertheless, Nelson-Barr models present several problems. On the one hand, further symmetries are needed in order to enforce the required mass matrix pattern (some allowed renormalizable terms like $\eta \overline{q}_L q_R$ or $H \overline{Q}_{L} {q}_{R}$ need to be forbidden). Furthermore, the vevs of the different complex scalars need to be adjusted to reproduce a large CKM phase and introduce a new hierarchy problem. Finally and most importantly, even if no $\theta$-term is present at tree level, loop contributions to $\theta$ can be large, requiring sophisticated matter content in order to control them.  

Analogously to the Nelson-Barr mechanism, models in which parity is spontaneously broken have also been considered  \cite{Babu:1989rb,Barr:1991qx,Mohapatra:1995xd,Kuchimanchi:1995rp,Mohapatra:1996vg}
. Indeed the $\theta$-term violates both P and CP while conserving C, so by constructing left-right symmetric models where P is spontaneously broken one can also address the strong CP problem. Typically these kind of models require new flavour structure that, similarly to Nelson-Barr models, induce important contributions to $\theta$ at loop level.

\subsection{Peccei-Quinn mechanism}
\label{Subsec: Peccei-Quinn mechanism}
One of the most elegant and simple solutions to the Strong CP problem was propossed by Peccei and Quinn in Ref.~\cite{Peccei:1977hh,Peccei:1977ur}. It consists on introducing a new abelian symmetry, the Peccei-Quinn symmetry $U(1)_{\text{PQ}}$, that is exactly conserved at the classical level but has a mixed anomaly with QCD,
\begin{equation}
\delta \mathcal{L}=\beta\,\partial_{\mu} J^{\mu}= \beta  \frac{\alpha}{8\pi}G_{\mu \nu} \widetilde G^{\mu \nu}\,,
\label{Eq: PQ anomaly}
\end{equation}
that explicitely breaks the symmetry at the quantum level.
As a consequence, this transformation of the fields allows to reabsorb completely the $\theta$ parameter from the Lagrangian, rendering it unphysical and solving the Strong CP problem. In addition, this PQ symmetry is spontaneously broken at a scale $f_a$ giving rise to the existence of a Goldstone boson, the axion \cite{Weinberg:1977ma,Wilczek:1977pj}. Due to the explicit PQ breaking by the anomaly, the axion acquires a non-zero mass constituting a pseudo-Goldstone Boson.

One of the most model-independent properties of the axion is that it couples to the QCD anomalous term as a consequence of \cref{Eq: PQ anomaly},
\begin{equation}
\mathcal{L}=\frac{a}{f_a}  \frac{\alpha}{8\pi}G_{\mu \nu} \widetilde G^{\mu \nu}\,.
\label{Eq: axion GGdual}
\end{equation}
This coupling allows for another possible interpretation of the PQ solution in terms of the axion effective Lagrangian. As it was shown by Vafa and Witten \cite{Vafa:1983tf} by considering the Euclidean path integral,

\begin{equation}
e^{-VE(\theta)}=\int \left[d A_{\mu}\right] \operatorname{det}(\slashed D+M) 
 e^{-\left(\nicefrac{1}{4 g^{2}} \int d^{4} x\, G_{\mu \nu} G_{\mu \nu}\right)}
\,e^{\nicefrac{i \theta}{32 \pi^{2}} \int d^{4} x \,  G_{\mu \nu} \widetilde G_{\mu \nu}}\,,
\label{Eq:Vafa witten path}
\end{equation}
the QCD vacuum energy has a minimum for $\theta =0$. This can be easily shown by taking into account that all the terms in the Euclidean action are real except for the $\theta$-term,\footnote{The Euclidean action is real at $\theta=0$ only if there is no other source of CP violation. Although this is not stricktly true in the SM, we have already seen that the effects on $\theta$ of the phase of the CKM can be safely neglected. } 
%S_E=S_{\text{real}}+S_\theta$,
\begin{align}
e^{-VE(\theta)}&\leq \int \left[d A_{\mu}\right]\left| \operatorname{det}(\slashed D+M)  e^{-S_{\text{real}}}
\,e^{\nicefrac{i \theta}{32 \pi^{2}} \int d^{4} x \,  G_{\mu \nu} \widetilde G_{\mu \nu}}\right|\\
&= \int \left[d A_{\mu}\right] \operatorname{det}(\slashed D+M) 
 e^{-S_{\text{real}}}=e^{-VE(0)}
\label{Eq:Vafa witten path II}
\end{align}
Therefore $E(\theta\neq 0) > E(0)$. 
This is essential for the viability of axion solutions to the strong CP problem. Effectively, the coulping of \cref{Eq: axion GGdual} amounts to promoting the $\theta$-parameter to a dynamical field, the axion, or substituting  $\theta\to \theta +\frac{a}{f_a}$. Since $E(\theta +\frac{a}{f_a}) > E(0)$, the non-preturbative effects of the QCD vacuum will generate a potential whose minimum lies at $\theta +\frac{a}{f_a}=0$ and therefore forces the vev of the axion to correspond to the CP conserving minimum,
\begin{equation}
\theta_{\text{eff}}=\theta +\Big\langle \frac{a}{f_a}\Big\rangle =0
\end{equation}
% \begin{equation}
% e^{-VE(\theta)}=\int \left[d A_{\mu}\right] \operatorname{det}(\slashed D+M) 
%  e^{-\left(\nicefrac{1}{4 g^{2}} \int d^{4} x\, G_{\mu \nu} G_{\mu \nu}\right)}
% \,e^{\nicefrac{i}{32 \pi^{2}}(\theta +a/f_a) \int d^{4} x \,  G_{\mu \nu} \widetilde G_{\mu \nu}}
% \label{Eq:Vafa witten path}
% \end{equation}
As consequence, the strong CP problem is solved in any theory which generates the coupling in \cref{Eq: axion GGdual} of the anomalous QCD term with a pseudoscalar which posseses a shift symmetry $a\to a +\alpha f_a$ only broken by that anomalous term. For more about axions, \cref{Ch: The axion} is devoted to review the properties of this particle.
\subsubsection*{Massless up-quark solution}
The simplest solution to the strong CP problem would be for the up-quark to be massless \cite{tHooft:1976rip}. 
In that case, $\text { Arg\,(det } M)$ would vanish and it would be impossible to write a physical CP phase that does not depend on the field redefinitions. 
Ultimately this solution is no different from the PQ mechanism.
 The axial rotation of the massless up-quark $U(1)_A:\,u\to e^{i \beta\g^5}u$ is a classical symmetry of the Lagrangian but explicitly broken by the QCD anomaly, see \cref{Eq: axial anomaly mass term} for $m=0$. Thus this symmetry is a perfectly valid PQ symmetry. Furthermore this symmetry is also spontaneously broken by the quark condensates upon confinement giving rise to a pseudo-Goldstone boson. One could identify the corresponding axion with the $\eta'$-meson.\footnote{Actually since the anomalous term badly breaks the $U(1)_A$ symmetry the $\eta'$ can not be considered a true pGB. However one can make this analogy by noting that the $\eta'$ is the lightest meson with the same quantum numbers as the axial current. }
One might wonder how a massless up-quark could be compatible with the observed meson masses. On the one hand, Mc Arthur and Georgi \cite{Georgi:1981be} showed that instantons can give an effective contribution to the up quark mass $m_u\sim m_dm_s/\lambda_{\text{QCD}}$ although the estimate is not reliable since the DIGA cannot be applied in the confining regime. On the other hand, it was shown by Manohar and Kaplan  \cite{Kaplan:1986ru} that second order terms in the chiral Lagrangian can generate an effective up quark mass that is also proportional $m_u\propto m_sm_d$ while being compatible with the pseudoscalar meson masses. These two results made the massless up-quark solution very appealing since it does not require any extension of the SM. Nevertheless, this alternative is now ruled out by lattice QCD results that show that the up quark has non-zero mass \cite{Gasser:1982ap,Nelson:2003tb,Aoki:2016frl,Frison:2017mod,Frison:2016rnq}.


\section{Why there is no Weak CP problem?}
Before finishing this chapter on the Strong CP problem it is interesting to comment on the reason why there is only a strong CP problem but not an electroweak or electromagnetic one. One can also write the topological terms for the electroweak gauge group of the SM $SU(2)_L\times U(1)_Y$,
\begin{equation}{}
\mathcal{L}_{\cancel{\mathrm{CP}}}=\theta_{\text{QCD}} \frac{\alpha_{s}}{8 \pi}  G_{\mu \nu} G^{\mu \nu}+
\theta_W \frac{\alpha_{W}}{8 \pi}  W_{\mu \nu} W^{\mu \nu}+
\theta_Y \frac{\alpha_{s}}{8 \pi}  B_{\mu \nu} B^{\mu \nu}\,.
\end{equation}
 All three terms correspond to total derivatives, but we showed in the previous sections that in the case of QCD the vacuum contains non-trivial configurations for which the integral in the boundary does not vanish, giving rise to observable effects. For the case of $U(1)_Y$, the vacuum does not contain such non-trivial configurations since the third homotopy group of the abelian group is trivial $\pi_3(U(1))=0$. As a consequence the corresponding $\theta_Y$-term has no physical impact.

 For the case of $SU(2)_L$, the sitauation is a bit more involved. Altough non-trivial maps from the sphere at infinity to the gauge group  can be constructed $\pi_3(SU(2))=\mathbb{Z}$, there are no exact instanton solutions since the theory is spontaneously broken. Still, as we showed in \cref{Sec: constrained instantons} there are approximate solutions of the Euclidean theory called constrained instantons that could generate a non-trivial vacuum. However, once fermions are taken into account the situation changes. As a consequence of $SU(2)_L$ gauge bosons interacting only with left-handed currents, both the baryon and lepton number current are anomalous,
 \begin{equation}
 \partial_{\mu} J_{\mu}^{B}=\partial_{\mu} J_{\mu}^{L}=\frac{\alpha_{W}}{4 \pi} W_{\mu \nu} W^{\mu \nu}\,.
 \end{equation}
Thus via a BN rotation the $\theta_W$ can be reabsorbed from the Lagrangian leaving no physical consequence. In other words, baryon (or lepton) number symmetry is the PQ symmetry of the EW topological term since it is classically conserved and explicitely broken solely by the EW anomaly. 




==> Chapters/zChapter3BAK/Chapter3bak.tex <==
%!TEX root = ../../Thesis.tex


\chapter{Holographic complexity of cosmological singularities}
\label{ch:capitulo4}

\section{Introduction} 


\noindent

From the origin of the universe to the interior of black holes, spacetime singularities seem to be present in some of the less understood phenomena within the field of fundamental physics. Not only they constitute one of the most misterious features of the theory of General Relativity, but also signal the very breakdown of it, calling for a UV completion able to resolve such singularities at distances below the Planck scale. Despite the success of perturbative string theory in the description of some timelike singularities, \comm{(through the expedient of exhibiting extra light degrees of freedom localized at the  singular locus)} much less is understood about the most realistic case of the spacelike ones, for which strong gravitational dynamics is believed to be needed.

Very broadly, there are two traditions regarding the interpretation of spacelike singularities: either they must be `resolved' so as to restore some type of  evolution across the singularity, or they must be accepted as  true `spacetime terminals'. To the extent that the black hole singularity is a general guide, the second option is preferred in modern discussions based on holography as the fist one putatively violates the entropic bounds\comm{. On the other hand, the straightforward application of holographic ideas requires an identification of appropriate AdS/CFT boundaries or at least some notion of holographic screen}. On the other hand, even within the realm of the well known benchmark examples of AdS/CFT, the search for a detailed mapping of the singularity in terms of the boundary degrees of freedom has been unsuccessfull. The ostensible obstructions to extend the so called `bulk reconstruction' procedure behind spacetime horizons \cite{Papadodimas, Harlowbulk} seems to render this problem both technically and conceptually non-trivial, hindering the search for useful CFT quantities that could describe or even diagnose the presence of bulk singularities.

A remarkable exception to this, however, is provided by AC complexity, which enjoys a quantitatively important contribution coming directly from the singularity through the evaluation of the YGH term. On the one hand, we might be suspicious of the validity of such contribution, as this is a term in the low-energy effective action that shoud be corrected in the gravitational strongly coupled regime (cf. \cite{Nally}). On the other hand, we are instructed to take this contribution seriously down to its precise dependence on coefficients, as this is crucial for the claimed uniformity of the growth law (\ref{CArate}) for AdS black holes in various dimensions, large and small. In a similar vein, the contribution (or lack of it) of the YGH term at the singularities is crucial for the `non-computing' behavior in various  systems, such as those studied in section \ref{sec:noncomp}.
  
These considerations suggest that holographic complexity is actually the piece of the holographic dictionary which most efficiently `sees' the properties of the singularities, a fact that encourages us to explore a broader phenomenology, seeking to associate holographic measures of quantum complexity to states which are linked to spacelike singularities by time evolution. This program was initiated in previous work \cite{BarbonRabinoComplexity, rabinonew} by the analysis of certain cosmological singularities with controlled AdS/CFT embedding. Here we seek to provide quasilocal notions of complexity which may be abstracted from particular AdS/CFT constructions, and  therefore   having a larger degree of generality. \comm{While we use the volume-complexity (VC) proposal \cite{SusskindEntnotEnough} as a heuristic guide, our discussion is tailored to the more covariant action-complexity (AC) proposal \cite{SusskindCAcorto, BrownSusskindAction}. }


The connection between spacetime singularities and complexity has a long history, going back to the occurrence of classical chaos in generic cosmological singularities   \cite{misner, BKL,BKL2,BKL3} (see \cite{libro} for  a recent review.) and other efforts to classify the different nature of singularities in the quest to seek for a gravitational definition of an `arrow o time' \cite{Penrose}. As we will see, holographic complexity provides a language in which some of these ideas can be realized in a precise way.



This chapter is organized as follows. In section \ref{sec:quasilocal} we lay down our setup and motivate the definition of the notion of `terminal holographic complexity', a new variant of the AC prescription which is well adapted to isolate the complexity of generic spacetime singularities. In section \ref{sec:locking} we investigate the universality properties of this quantity in some  examples of singularities admitting a completely analytic treatment. In section \ref{sec:local} we discuss a coarse-graining procedure that can isolate a local contribution to complexity at the singularity and speculate about the resemblance with older proposals for such local measures of gravitational complexity. Finally, in section \ref{sec:conclusions} we offer some conclusions and outlook for plausible generalizations. 





\section{A quasilocal AC ansatz for terminals}
\label{sec:quasilocal}
\noindent

In the benchmark model provided by the eternal black hole spacetime, the central object of interest for the VC ansatz is the extremal codimension-one surface $\CS_\infty$ shown in Figure \ref{fig:sigmainf}. This surface maximizes the volume locally and it lies entirely within the black hole interior, i.e. the past causal domain of the singularity.  


The growth of complexity within the VC ansatz can be seen as the result of gradually accessing an increasing portion of $\CS_\infty$. More precisely, the portion of the extremal surface ${\CS}_t$ which has a significant contribution to time dependence  can be analyzed approximately as composed of two parts: a subset of $\CS_\infty$ with volume proportional to $t$, and a transition surface at the horizon, whose contribution to the complexity is of order $S$, the entropy of the black hole. Let us denote by ${\CS}'_t$ this, loosely defined,  `subtracted' surface as indicated in Figure \ref{fig:sigmainf}. 

\begin{figure}[h]
$$\includegraphics[width=10cm]{sigmainf.eps} $$   
\begin{center}
\caption{\emph{  On the left, the codimension-one asymptotic surface ${\cal S}_\infty$, accounting for the total complexity `flowing' into the black-hole singularity $\CS^*$. On the right, the subtracted codimension-one surface ${\CS}'_t$ which accounts for the time-dependence of VC complexity in the eternal black hole geometry. }\label{fig:sigmainf}}
\end{center}
\end{figure} 


Once we decide to focus on ${\cal S}'_t$ and its asymptotic limit $ {\cal S}_\infty$, we may consider  versions of these quantities for any terminal set $\CS^*$ (which may in particular be a proper  subset of a wider one.) The reason is that the analog of ${\cal S}_\infty$ always exists given any spacelike terminal set $\CS^*$ and its associated past domain of dependence $D^-(\CS^*)$  (see Figure \ref{fig:DS}.) Since the volume is positive and the past boundary of $D^- (\CS^*)$ is null, the extremal surface is either a local maximum of volume or it coincides with $\CS^*$ in a degenerate case. The first situation occurs when $\CS^*$ is a standard singularity of the kind we encounter at black holes and cosmological crunches in General Relativity, since the volume of spatial slices vanishes at such singularities.

 \begin{figure}[h]
$$\includegraphics[width=10cm]{domains.eps} $$   
\begin{center}
\caption{\emph{Generic terminal set $\CS^*$ (in red) and its past domain of dependence $D^-(\CS^*)$ and causal past $J^-(\CS^*)$ .  }\label{fig:DS}}
 \end{center}
\end{figure} 



A more covariant version of $\CS_\infty$ and ${\CS}'_t $ could be obtained by adapting the AC ansatz to this situation (cf. Figure \ref{fig:c1}.) Since ${\cal S}_\infty$ is the extremal surface on $D^-({\cal S}^*)$, the natural AC version of the full  terminal complexity of the set ${\cal S}^*$ is the on-shell action 
\begin{equation}\label{fullc}
\CC[{\cal S}^*]  =  I\left[D^-({\cal S}^*)\right]
\;,
\end{equation}
evaluated over the set $D^- ({\cal S}^*)$. Since this definition  only makes reference to the terminal set ${\cal S}^*$ we regard this notion of complexity as `quasilocal' and will often denote it as such. 




 \begin{figure}[h]
$$\includegraphics[width=5cm]{c1.eps} $$   
\begin{center}
\caption{\emph{  The total VC complexity flowing into the singular set ${\cal S}^*$ is the volume of the asymptotic surface ${\cal S}_\infty$. Its AC analog is the on-shell action integrated over the past domain of dependence $D^- ({\cal S}^*)$.  }\label{fig:c1}}
 \end{center}
\end{figure} 


 \begin{figure}[h]
$$\includegraphics[width=5cm]{c2.eps} $$   
\begin{center}
\caption{\emph{  The WdW patch ${\cal W}_t$, associated to the cut-off surface ${\cal S}'_t$, intersects the singularity at ${\cal S}^*_t$. }\label{fig:c2}}
 \end{center}
\end{figure} 




Next, a  notion of `time-dependence'  can be defined by considering a WdW patch anchored roughly at the exit points of the cut-off surface ${\cal S}'_t$, as indicated in  Figure \ref{fig:c2}. A more invariant definition can be obtained by noticing that these WdW patches are
nested into one another as time increases. For sufficiently `late' WdW patches, this `nesting' extends to the intersections of the WdW patches with the singular set. This suggests that  we may use the nested singular subsets as a starting point in the definition of the WdW nested family. To be more precise, let us pick  a sequence $ \lbrace {\CS}^*_u  \rbrace $ of terminal subsets labelled by $u$ , ordered by inclusion in the sense that
\begin{equation}
{\CS}^*_u \subset {\CS}^*_{u'}  \;, \; {\rm for}\;\; u<u'\;,
\end{equation}
and  converging to 
the full terminal set $\CS^*$ as $u\rightarrow u_*$, we can consider a set of WdW patches ${\cal W}_u$, defined as the intersection between $D^- (\CS^*)$ and 
the causal past of ${\CS}^*_u$, 
\begin{equation}\label{wdwu}
{\cal W}_u = J^- ({\CS}^*_u) \cap D^- ({\CS}^*)\;.
\end{equation}



 
For any given ${\cal W}_u$, its Cauchy surfaces $\Sigma_u$  have a common codimension-two boundary ${\cal V}_u = \partial \Sigma_u$ (cf. Figure \ref{fig:wdwu},) which would hold the `holographic data' for ${\cal W}_u$. For example, ${\cal V}_u$ is a spatial section of the event horizon when $\CS^*$ is a black-hole singularity.   Therefore, we would like to interpret the `area' of ${\CV}_u$ in Planck units \footnote{ We henceforth refer to  codimension-two volumes as `areas'.} as a measure of the effective number of holographic degrees of freedom `flowing' into the terminal subset ${\CS}^*_u$, assigning therefore the entropy

\begin{equation}
S= \dfrac{{\rm Area}[{\CV}_u]}{4 G}\, ,
\end{equation}

to the singular subset.

In defining the WdW patches ${\cal W}_u$ we may give privilege to the `anchors', namely the codimension-two sets ${\cal V}_u$, or alternatively we may consider  the nested family ${\cal S}^*_u$, as more fundamental. These two constructions  are not completely equivalent, since the WdW patch anchored at ${\cal V}_u$ may fail to intersect ${\cal S}^*$ at sufficiently `early times'. In this paper
we are more interested in the asymptotic `late-time' behavior in which ${\cal W}_u$ does have a non-trivial boundary component at the singularity. Therefore, we tacitly adopt in what follows the nesting construction of the WdW patches and we will often refer to the
associated complexity measures as `nesting complexity'. 

With the previous definitions, we are led to the following definition of nesting complexity associated to the given family of WdW patches ${\cal W}_u$, 
\begin{equation}
\label{terminaldef}
\CC^*(u)=  \,I[{\CW}_u]  \;,
\end{equation}
where $I[{\CW}_u]$ denotes the on-shell gravitational action, now integrated over the WdW patch ${\cal W}_u$. Once this nesting complexity is defined, we can now recover the notion of `total complexity flow' into the singularity, which was loosely defined in (\ref{fullc}), as the asymptotic limit of the nesting procedure. More precisely, we have
\begin{equation}\label{toal}
\CC[{\cal S}^*] =  \lim_{u\to u_*} \CC^*(u) \;,
\end{equation}
It is important to notice that, when considering singular subsets ${\cal S}_u^*$, the nesting complexity $\CC^*(u)$ is {\it different} from the `total complexity'   $\CC[{\CS}^*_u]$ flowing into ${\cal S}^*_u$, as shown in Figure \ref{fig:nest}. In other words,  
we regard $\CC[\CS^*]$ as the AC-analog of ${\CS}_\infty$, (cf. Figure \ref{fig:c1},)  and $\CC^*(u)$ as the AC-analog of ${\CS}'_t$, (cf. Figure \ref{fig:c2}.) 

\begin{figure}[h]
$$\includegraphics[width=8cm]{wdwu.eps} $$   
\begin{center}
\caption{\emph{ The WdW patch ${\CW}_u$ (in yellow), associated to a given ${\CS}^*_u$ subset (in black) of the full terminal set $\CS^*$ (in red).  The codimension-two set ${\CV}_u$ is the (possibly disconnected) boundary of Cauchy surfaces $\Sigma_u$ for ${\CW}_u$. }\label{fig:wdwu}}
 \end{center}
\end{figure} 




\begin{figure}[h]
$$\includegraphics[width=6cm]{nest.eps} $$   
\begin{center}
\caption{\emph{ The difference between $\CC^*(u)$ and $\CC[{\cal S}^*_u] $ as determined by the different domains of integration. }\label{fig:nest}}
 \end{center}
\end{figure} 



\subsection{Technical aside: action prescription}
\label{sec:actionprescription}

Before entering into the phenomenology of terminal complexity, we must clarify some technical points. In particular, the gravitational action for the WdW patch is not unique, and some prescriptions are to be setlled down. As shown in \cite{Poisson}, the Einstein-Hilbert action for some patch $\CW$ with arbitrary boundaries can be defined with the following prescription for codimension-one and codimension-two boundary terms

\begin{eqnarray}
\label{masterformula}
16 \pi G \, \tilde{I}[\CW] &=& \int\limits_{ \CW} \text{d}^{d+1}x \,\sqrt{-g}\,(R-2\Lambda + \mathcal{L}_m) \\ \nonumber &+& 2 \sum\limits_{\CT_i} \int\limits_{ \CT_i} \text{d}^dx \,K   + 2 \sum\limits_{\CS_i} \sgn(\CS_i)\int\limits_{ \CS_i} \text{d}^d x \,K  \\ &-&  2 \sum\limits_{\CN_i} \sgn(\CN_i)\int\limits_{ \CN_i} \text{d}^dx \,\text{d}\lambda \,\hspace{0.1cm}\kappa  +2 \sum\limits_{j_i} \sgn(j_i)\oint\limits \text{d}^{d-1}x \,\alpha_{j_i} \, , \nonumber
\end{eqnarray}
where in this expression

\begin{itemize}
\item $\CT_i$, $\CS_i$ and $\CN_i$ are respectively the timelike, spacelike and null boundaries of the WdW patch and $K$ are the traces of the corresponding extrinsic curvatures for the first two cases. For the null boundaries, $\lambda$ represents an arbitrary parameter on null generators of $\CN_i$, with $\kappa$ the surface gravity associated to $\CN_i$ in this parametrization. The signs for the null and spacelike boundary contributions are defined depending on the relative location of the boundary to the WdW patch as follows $$ \text{sgn} \left( \raisebox{0pt}{\includegraphics[height=0.26cm]{spacelikesign.pdf}} \right)=\text{sgn} \left( \raisebox{-5pt}{\includegraphics[height=0.5cm]{null2.png}} \right)=\text{sgn} \left( \raisebox{-5pt}{\includegraphics[height=0.5cm]{null3.png}} \right)=-\text{sgn} \left( \raisebox{-2pt}{\includegraphics[height=0.26cm]{spacelikesign2.pdf}} \right)=-\text{sgn} \left( \raisebox{-5pt}{\includegraphics[height=0.5cm]{null4.png}}\right)=-\text{sgn} \left( \raisebox{-5pt}{\includegraphics[height=0.5cm]{null1.png}} \right)   =1.$$

\item $j_i$ are the codimension-two junctions between boundary components. For those joints that are formed by at least one null boundary, the form of the integrand in \eqref{masterformula} is given by

\begin{equation}
\alpha_{j_i} = 
\begin{cases}
\log |k_\mu n^\mu| \\
\log |k_\mu s^\mu|\\
\log |\frac{1}{2}k_\mu \bar{k}^\mu|,
\end{cases}
\end{equation}

where $k^\mu$ and $\bar{k}^\mu$ are taken to be the future directed vectors tangent to the null surfaces and $n^\mu$ ($s^\mu$) is the future-directed (outward-directed) unit normal to the spacelike (timelike) surface. For such terms the signs $\sgn(j_i)$ are simply given by the product of the surfaces signs. Joints that are formed only by spacelike and timelike boundaries have a different set of rules that we will not cover here as they do not appear on WdW patches (see \cite{Poisson} for a full discussion of all possible joint actions).
\end{itemize}


The boundary terms in \eqref{masterformula} require special consideration. As we see, the boundary piece of the action is given by a sum of contributions from  codimension-one and codimension-two components of the boundary $\partial {\cal W}$. The non-null codimension-one pieces and their joints  are given by the standard York--Gibbons--Hawking (YGH) term and a set of well understood joint contributions.  On the other hand, some formal choices are necessary in the  presence of null codimension-one pieces as the freedom to choose the parametrization of null generators renders the on-shell action a gauge-dependent quantity. The physics behind these choices remains somewhat unclear (see for example the considerations in \cite{Poisson, Ross, MyersFormation, WhichAction, SusskindJT},) and different prescriptions can lead to qualitatively different behaviours for the action and its dynamics. Accordingly, it becomes a central issue to settle for one of such prescriptions in order to perform any sort of detailed study of complexity growth phenomenology. A way to circunvent this problem was pointed out in \cite{Poisson} where it was shown that it is possible to enforce reparametrization invariance of the gravitational action by the addition of an extra counterterm depending on the expansion of codimension-two sections along the null boundaries
\begin{equation}
\label{expansioncounterterm}
\Theta = \partial_\lambda \,\log\,\sqrt{\gamma}
\;. 
\end{equation}
We shall refer to this addition as the  expansion counterterm:
\begin{equation}
\label{Ict}
I_{\Theta} = \sum\limits_i\dfrac{\text{sgn}(N_i)}{8\pi G} \int\limits_{N_i}  \text{d}\lambda\, \text{d}^{d}x \;\sqrt{\gamma}\; \Theta \;\log(\ell_\Theta\, \cdot |\Theta|).
\end{equation} 


The appearance of the new length scale $\ell_\Theta$ is interesting. It represents a qualitatively new feature of AC complexity which, as we will see, activates itself  precisely in cases where the entropy has a dynamical behaviour and the effective Hilbert space supporting the singularity  changes its dimension. The presence of $I_\Theta$ has been regarded as necessary to  guarantee the positivity of complexity \cite{Ross} as well as the correct black hole complexity dynamics from collapsing geometries and the verification of the switchback effect \cite{VaidyaI, VaidyaII, WhichAction}. Its precise meaning in microscopic treatments inspired by the notions of circuit complexity remains however quite mysterious (cf. \cite{JeffersonMyers, Myersmixed, Myerscoherent, MyersTFD }). 

In the following we will adopt such prescription for our terminal complexity, meaning that our definition \eqref{terminaldef} is to be understood with
\begin{equation}\label{def}
I[{\cal W}_u] =  \tilde{I} [{\cal W}_u] + I_\Theta [{\cal W}_u]\;,
\end{equation}
with $\tilde{I}$ and $I_\Theta$ given by \eqref{masterformula} and \eqref{Ict} respectively. A careful evaluation of the boundary terms and counterterm will in fact be crucial for our purposes, since we are precisely interested in situations with non-trivial null-expansion.


\section{Entropic locking of terminal complexity}
\label{sec:locking}

\noindent
The persistence of complexity growth well after the entropy of the black hole has stabilized is considered to be a fundamental property. More precisely, since the conjectured bound on complexity is non-perturbative in $1/S$, the bulk expansion parameter, the total AC/VC complexity accumulated by an eternal black hole is infinite when computed in leading orders, in correspondence to the infinite volume and action of the black hole interior.

Away from the benchmark example of a static black hole, however, neither the positive growth of complexity nor its decoupling from the entropy dynamics are self evident at all, begging the question of whether these features are to hold for more generic solutions enjoying non-trivial dynamics. As the black hole possess a constant entropy, we may in fact interpret the terminal AC as a measure of the purely infrared contribution to complexity, including only those degrees of freedom which are actually involved in the holographic emergence of the black hole interior. Considering time-dependent UV/IR thresholds in AdS/CFT constructions, we may generalize this setup to situations with dynamical entropy, interpreting the IR Hilbert space as enjoying a time-dependent dimension and associating a quasilocal terminal complexity to them.

More precisely, given a singular spacetime of the type shown in Figure \ref{fig:terminalcomplexity},  with a terminal singularity ${\cal S}^*$ and a horizon bounding the past domain of dependence $D^-({\cal S}^*)$, we can ask how the accumulated complexity compares with the entropy. The formal definitions laid down in section \ref{sec:quasilocal} allow us to perform a sharp comparison, exploring the phenomenomenology trough a set of qualitatively different dynamical examples in which ${\rm Area}({\cal V}_u)$ varies strongly as $u\rightarrow u_*$ on approaching the singularity. Our results indicate that the rate of complexity growth is generically dominated by the finite-size effects in the Hilbert space, namely the rate of variation of the entropy, rather than the standard process of `entanglement weaving' which leads to linear complexity growth in black holes. 



\begin{figure}[h]
\begin{center}
\includegraphics[width=6cm]{generic_growth.pdf} 
\caption{\emph{ The WdW patch $\CW_u$ (in yellow), parametrized by a null coordinate on the boundary of the singularity's past domain of dependence. Entropy is measured by the volume of ${\cal V}_u$ and complexity is measured by the action of ${\cal W}_u$.
This construction is modified in the obvious manner under time reversal.}}
\label{fig:terminalcomplexity}
\end{center}
\end{figure} 


More specifically, this `entropic locking' of complexity is found in two different situations  which illustrate qualitatively different dynamics as classified by the behaviour of its entropy. Our choices are motivated by the ability to compute exactly the complexity on terminal WdW patches using the specific formula \eqref{terminaldef},  but also by our interest in exposing as much as possible the contrast between entropy and complexity when referred to cosmological singularities. One case corresponds to expanding bubbles of Coleman-de Luccia  type, engineered in concrete AdS/CFT scenarios.  Here both the terminal AC complexity and the entropy diverge at the singular locus and we are interested in the relative rates of divergence. The second example is a portion of  the Kasner spacetime, which is known to locally approximate any spacelike singularity  in GR. In this case the entropy vanishes and the terminal AC complexity approaches a constant. 

Our main result is that, as the singularity is approached, $u \rightarrow u_*$, in both classes of examples,  the  terminal AC growth is completely controlled by that of the entropy  $S$ through a law of the form
\begin{equation}
\label{law}
 \delta { \cal C^*} =  a\, \delta S+\dots  \,
\;,
\end{equation}
with $a$ a non-universal constant. Here, $S={\rm Vol} ({\cal V}_u)/4G$ and the dots stand for  $u$-independent contributions or subleading terms as $u\rightarrow u_*$.  More specifically, for the case of expanding bubbles we find the sign of the $a$ coefficient depending on the counterterm scale $\ell_\Theta$, implying that a positive rate of complexity growth  actually requires  picking a sufficiently large value of this scale, as measured in units of the AdS radius of curvature. In the Kasner case, the positivity of the coefficient $a$ is guaranteed by the weaker condition $\LL \gg \ell_{\text{Planck}}$ yielding a decreasing complexity as the effective Hilbert space is reduced.


Before embarking in our tour of examples, we would like to comment briefly on the relation to previous work. In \cite{BarbonRabinoComplexity}  the VC complexity was estimated for a number of cosmological singularities which are naturally embedded into concrete AdS/CFT constructions. In these examples it was found that a regularized version of the VC complexity was monotonically {\it decreasing} on approaching the singularity, in contrast with our statement here for the cuasilocal complexity. A similar behavior was obtained for the AC ansatz in the same examples by \cite{rabinonew}. The reason for this apparent discrepancy is simply that the full complexity computed in \cite{BarbonRabinoComplexity} is dominated by UV contributions to the VC ansatz, and these are highly dependent on the particular details of the embedding into asymptotically AdS geometries. For instance, some of the examples are based on singular CFT metrics which shrink to zero size, and others involve expanding domain walls in the bulk. In the first case it is natural that the UV contribution to complexity should have a negative derivative in time, as corresponds to a shrinking Hilbert space on the full CFT. In the second case, a time-dependent conversion between UV and IR degrees of freedom is introduced in the CFT by switching on a relevant operator with a time-dependent coupling, and the c-theorem explains why the UV again dominates the balance.    Therefore, there is no contradiction since the two monotonicity statements refer to different quantities. The positive monotonicity of the quasilocal complexity defined here (by restriction of the AC/VC ansatz to the interior of $D^- ({\cal S}^*)$,) is compatible with the negative monotonicity of the full complexity, particularly when  the latter is dominated by a strong UV time-dependence.  


\subsection{Vacuum terminals with divergent entropy}

\noindent



The primary example is that of a singularity inside an expanding bubble embedded in an ambient AdS spacetime. Such solutions look like standard crunching cosmologies of FLRW type, where the singularity eventually crunches the whole AdS spacetime in a finite time as measured by the asymptotic global time. The boundary of the bubble has an acceleration horizon which serves as the boundary of the past causal domain $D^- ({\cal S}^*)$. As a result, the entropy of this crunch singularity is infinite.

In order to rely on analytic methods,\footnote{For a mereley cosmetic reason, we adopt only in this section the convention that $d$ always stands for the dimensionality of $\CV_u$, i.e. we will work in AdS$_{d+2}$ spacetimes.} we first consider the `topological cruch' model (cf. \cite{Banados, maldapim, BarbonRabinoCrunches}),   which describes a time-dependent compactification of pure AdS$_{d+3}$ with topology AdS$_{d+2} \times {\bf S}^1$, where the ${\bf S}^1$ shrinks to zero size in finite boundary time, producing a spacelike singularity in the interior as shown in Figure \ref{fig:tc}. A holographic interpretation of this model uses a CFT$_{d+2}$ on a spatial manifold with topology $ {\bf S}^{d} \times {\bf S}^1$, where  the sphere is static and the circle shrinks to zero size in finite time. A conformally related description is that of the same CFT on a fixed-size circle, times a de Sitter spacetime. 



\begin{figure}[h]
$$\includegraphics[width=8cm]{topological.pdf} $$   
\begin{center}
\caption{\emph{ The causal structure of the topological crunch singularity and its associated WdW patch. }
\label{fig:tc}}
 \end{center}
\end{figure} 




In the FLRW patch of the $AdS_{d+2}$ the metric for this model is given by
\begin{equation}
\text{d}s^2 = -\text{d}\tilde{t}^{\,2} +  \sin^2 (\tilde{t}\,) \,\text{d}{\bf H}_{d+1}^2 + \cos^2 (\tilde{t}\,) \,\text{d}\phi^2 \, ,
\end{equation}
where we have set the AdS scale to unity and also consider that to be the curvature scale of the boundary metric. The element $d{\bf H}_{d+1}^2$ stands for the unit metric on the $(d+1)$-dimensional Euclidean hyperboloid ,whereas the coordinate $\phi$ is the angle that parametrizes the compact circle ${\bf S}^1$. The time $\tilde{t}$ foliates the cosmology with sections of topology ${\bf H}_{d+1} \times {\bf S}^1$, producing a singularity $\mathcal{S}^*$ when the circle shrinks to zero size at time $\tilde{t}_*=\pi/2$.


In order to perform the required computations, it is useful to define null coordinates on $D^- ({\cal S}^*)$ as follows. First, we introduce a radial coordinate $\chi$ over ${\bf H}_d$ and a conformal time variable $\eta =2\tan^{-1} \left( e^{\tilde{t}/\ell}\right)$ over the AdS$_{d+1}$ factor, so that the metric is written in the form
 \begin{equation}\label{mc}
 ds^2 =\sin^2 (\tilde{t}\,) \left[ -d\eta^2 + d\chi^2 + \sinh^2 (\chi) \,d\Omega_{d}^2\right] +  \cos^2 (\tilde{t}\,) d\phi^2\;.
\end{equation}
Next, we  introduce null compact Kruskal coordinates  
\begin{eqnarray}
\tan u=  e^{\eta + \chi} \;, \qquad \tan v = e^{\eta - \chi} \, ,
\end{eqnarray}
for which we get the full analytic continuation of the metric in the form


\begin{equation}
\label{topmetric}
\text{d}s^2 =  \sec ^2(u-v) \left[ -4 \,\text{d}u \text{d}v + \sin ^2(u-v) \,\text{d}\Omega^2_{d} + \cos^2 (u+v)\, \text{d} \phi^2 \right].
\end{equation}

Considering now the set of nested WdW patches $\CW_u$ labeled by the null coordinate $u$, we are ready to calculate the different contributions to the on shell action from the prescription \eqref{masterformula}. As we will only care about asymptotic behaviors and not the exact full action, it will suffice to consider stripes $\delta \CW_u$ of thickness $\delta u$ for which computations render sensibly simpler results. The bulk action piece of such stripe is given by

\begin{eqnarray}
I_{\text{bulk}}[\delta \CW_u] &=& -\dfrac{(d+2)}{8 \pi G} \int\limits_{\delta \CW_u} \text{d}^{d+3}x \, \sqrt{-g} \\
&=& -\dfrac{2(d+2)V_\Sigma}{8 \pi G} \int\limits^{u+\delta u}_{u} \text{d}u  \int\limits_0^{\pi/2-u} \text{d}v \; \dfrac{\tan^d(u-v)}{\cos^3(u-v)}\cos(u+v)\,.
\end{eqnarray}
where $V_\Sigma$ stands for the area of the ${\bf S}^{d}\times {\bf S }^1$ manifold. Performing this integral and expanding around $u\sim u_*=\pi/2$ we can obtain the asymptotic limit for the bulk action growth

\begin{equation}
\dfrac{\text{d} }{\text{d}u} I_{\text{bulk}}[ \CW_u] \approx -\dfrac{V_\Sigma}{8 \pi G} \,\dfrac{2(d+2^{-d-1})}{d+1}\left( \dfrac{1}{u_*-u} \right)^{d+1}.
\end{equation}

In order to calculate the codimension-one boundary terms, we will choose to parametrize all null boundaries affinely, so that the extrinsic curvature vanishes and such contributions are identically zero. The only non-trivial YGH contribution will be that of the spacelike boundary at the singularity, which is located at $\tau \equiv v+u =\pi /2$. This term is given by
\begin{equation}
I_{\text{YGH}}[ \CW_u] = -\dfrac{1}{8 \pi G} \int\limits_{\CS^*_u} \text{d}^{d+2}x \,\sqrt{\gamma}\,K \, ,
\end{equation} 
where $\gamma$ is the induced metric on $\CS^*_u$ and the integrand is calculated using $\sqrt{\gamma} \, K = g_{\tau \tau}^{-1/2} \, \partial_\tau \sqrt{\gamma}$. Performing the integral again for the slab of thickness $\delta u$ we get the growth rate and its late time limit
\begin{equation}
\dfrac{\text{d} }{\text{d}u}I_{\text{YGH}}[ \CW_u]  = \dfrac{V_\Sigma}{8 \pi G} \dfrac{\tan^{d+1}(2u)}{\sin^{}(2u)}\approx \dfrac{V_\Sigma}{8 \pi G} 2^{-d-1}\left( \dfrac{1}{u_*-u} \right)^{d+1}.
\end{equation}
The only codimension-one contribution that is now left is that of the expansion counterterms \eqref{Ict}. Let us consider thus the WdW null boundaries, which will be given by constant $u,v$ hypersurfaces. For instance, we may start with the past boundary, given by the surface $N_- \equiv (u,0,\Omega_0, \phi_0)$, where the coordinate $u$ here will parametrize the geodesic. Introducing this curve into the geodesic equation, however, we can see that such parametrization is not affine, but rather has the following surface gravity
\begin{equation}
\kappa(u) = 2 \tan u \,.
\end{equation}
Following the standard procedure, we can find an affine parameter $\lambda_-$ from the relation
\begin{equation}
\dfrac{\text{d} \lambda_-}{\text{d}u} = \exp{\int\limits_0^u\kappa(\sigma) \, \text{d} \sigma}\, ,
\end{equation}
which for our case yields
\begin{equation}
\lambda_- = \dfrac{1}{\alpha_-} \tan u\,,
\end{equation}
and we have introduced a constant $\alpha_-$ that parametrizes the freedom to shift the affine parameter. From \eqref{topmetric} we can extract the determinant of the induced transverse metric as well as its expansion and express them in terms of $\lambda_-$
\begin{eqnarray}
\sqrt{\gamma} &=& (\alpha_-\lambda_-)^{d}\, ,\\
\Theta &=&  \dfrac{d}{\lambda_-}\, .
\end{eqnarray}
Feeding this into the counterterm definition \eqref{Ict} we get the contribution to the action
\begin{eqnarray}
\label{counterU}
I^-_{\Theta} &=& \dfrac{V_\Sigma}{8 \pi G} \int\limits_0^{\frac{1}{\alpha_-}\tan u}  \text{d}\lambda_- \, \alpha_- \,(\alpha_-\lambda_-)^{d-1}d \, \log \left(\LL \dfrac{d}{\lambda_-} \right) \\  
&=&\dfrac{V_\Sigma}{8 \pi d G} \tan ^{d}u \, (d \, \log (d \, \LL \, \alpha_- \cot u)+1)\,.
\end{eqnarray}
A similar procedure gives us the affine parameter for the future null boundary $N_+$
\begin{equation}
\lambda_+ = \dfrac{1}{\alpha_+} \tan (u-v)\, ,
\end{equation}
which yields
\begin{equation}
\sqrt{\gamma} = (\alpha_+   \lambda_+ )^{d} (\alpha_+  \lambda_+  \sin (2 u)+\cos (2 u)),
\end{equation}
\begin{equation}
\Theta = \frac{1}{\lambda_+ }\left(d+1-\frac{1}{\alpha_+  \lambda_+  \tan (2 u)+1} \right),
\end{equation}
and we can calculate the corresponding counterterm \footnote{Although this integral is analytically solvable, the result is rather cumbersome and not particularly illuminating. We omit therefore such explicit expression since we will only care about its late time expansion.}


\begin{eqnarray}
\label{counterV}
\scriptsize
I^+_{\Theta} &=&  -\dfrac{V_\Sigma}{8 \pi G} \int\limits^{\frac{1}{\alpha_+} \tan(2u-\frac{\pi}{2})}_{\frac{1}{\alpha_+} \tan u} \text{d}\lambda_+ \, \text{d}^{d+1}x \, \sqrt{\gamma} \,\Theta \,\log(\LL \,|\Theta|).
\end{eqnarray}
Finally, we must also calculate the contribution from the codimension-two joints of $\CW_u$. As the joint $N_+ \cap \CS^*_u $ has vanishing volume, the only one that will produce a non-trivial contribution is $\CV_u = N_- \cap N_+$. Following the rules on section \ref{sec:actionprescription}, the contribution from this joint is given by  
\begin{equation}
\label{Sjoints}
I_{\CV_u} =  -\dfrac{1}{8 \pi G} \oint\limits_{\CV_u} \text{d}^{d+1}x \, \sqrt{\sigma} \, \log | \tfrac{1}{2}k_+ \cdot k_- |\,  ,
\end{equation}
where $k_+$ and $k_-$ are respectively the null tangent vectors of the future and past boundaries. We choose these vectors to be
\begin{eqnarray}
k_+ &=& \alpha_+ (dT+dX)\,,\\
k_- &=& \alpha_- (dT-dX)\,,
\end{eqnarray}
so that they satisfy $k_{\pm} \cdot \partial_T=\alpha_{\pm}$ and $\alpha_{\pm}$ are normalization constants. Substituting these values into \eqref{Sjoints} we get the contribution of the joint
\begin{eqnarray}
\label{jointint}
I_{\CV_u} &=& -\dfrac{1}{8 \pi G} \log \left(\alpha_+ \, \alpha_-   \dfrac{\cos^2u}{2}\right) \oint \text{d}^{d+1}x \, \sqrt{\sigma}  \\ &=& \nonumber -\dfrac{V_\Sigma }{8 \pi G}\log \left(\alpha_+ \, \alpha_-   \dfrac{\cos^2u}{2}\right)  \tan^{d} u\, .
\end{eqnarray}

We observe that the dependence on $\alpha_\pm$ cancels out when \eqref{counterU}, \eqref{counterV} and \eqref{jointint} are added up, and accordingly we can set them to 1 in these expressions. Collecting all results for a late time expansion $u \sim u_*$, we get the following  behavior for the contributions
\begin{eqnarray}
I_{\text{bulk}} &\approx & -\dfrac{S}{\pi d} \left( \dfrac{d+2^{-d-1}}{d+1}\right)\, , \label{topbulk}\\ 
I_{\text{YGH}} &\approx & \dfrac{S}{\pi d} \times 2^{-d-1}\, ,\label{topYGH} \\
I^-_{\Theta}  &\approx & \dfrac{S}{2\pi d}\left[ 1+ \log\left(\dfrac{V_\Sigma}{4G} \right)+d\log\left(d\, \LL\right)-\log S\right], \\
I^+_{\Theta}  &\approx & \dfrac{S}{2\pi d} \left[ f(d) + \log\left(\dfrac{V_\Sigma}{4G} \right)+d\log\left(d\,\LL\right)-\log S \right], \\
I_{\CV_u}  &\approx & \dfrac{S}{2 \pi d} \left[d\log(2)- 2 \log\left(\dfrac{V_\Sigma}{4G} \right)  +2 \log S \right], 
\end{eqnarray}
where we are dropping terms in fractional powers of the entropy $S$ along the horizon, defined as  
\begin{eqnarray}
\label{entropytop}
S &=& \dfrac{1}{4 G} \oint  \text{d}^{d+1}x \, \sqrt{\sigma}  \\ &=& \nonumber \dfrac{V_\Sigma }{4 G} \tan^{d} u \approx \dfrac{V_\Sigma}{4 G}\left( \dfrac{1}{u_*-u} \right)^{d},
\end{eqnarray}
and keeping only the leading and next-to-leading contributions to the action. The coefficient $f(d)$ is an $\CO(1)$ positive constant given by
$$\scriptstyle  (d+1)f(d)=  \left(d^2+d-1\right) \, _2F_1\left(1,d;d+1;2+\frac{2}{d}\right)-d^2+2 (d+1) d \left(\coth ^{-1}(d+1)-\, _2F_1\left(1,d+1;d+2;2+\frac{2}{d}\right)\right)+2^{-d} \, _2F_1\left(1,d;d+1;1+\frac{1}{d}\right).$$


After adding up all contributions, we can see that the $S\log S$ divergence cancels out, yielding a total late-time complexity dynamics linear in the entropy

\begin{equation}
 \CC^* \approx   a\, S
\end{equation}
with
\begin{equation}
a= \dfrac{1}{\pi d} \left[\dfrac{-d-2^{-d-1}}{d+1} +  2^{-d-1} + \dfrac{1}{2} \left(1+f(d)+d\log (2) \right) +d\log \left( d\, \LL\right) \right].
\end{equation}


As we see, the complexity growth is fully controlled by that of the entropy, diverging as measured by any null coordinate along the horizon. The sign of such growth however will depend on the coefficient, which is essentially controlled by the size of $\LL$,  yielding a positive rate when $\LL \gtrsim 1$ for any dimension.\\

\comm{If we choose on the other hand to single out only the geometric complexity $\CC_g$, we can see from \eqref{topbulk} and \eqref{topYGH} that we find again a linear relation $\CC_g = \bar{a}\, S$ with $\bar{a}$ a negative coefficient, evidencing the need of the boundary terms and counterterms to render a positive growth. COMENTAR LO DEL PRIMER PAPER?}




It would be interesting to generalize this result to more general solutions with expanding horizons. The need to consider scalar fields with non-trivial potentials generally prevents us from a completely analytic treatment. However, we can offer evidence that the result found is quite robust by examining a similar situation in the so-called thin-wall approximation. Suppose that the bubble has a very narrow outer shell, so that we can describe it as a thin wall expanding into AdS$_{d+2}$, with a de Sitter induced metric. In this case the singularity can be regarded as a null future-directed surface emerging from the boundary  impact time at $t=t_*=\pi $  (see Figure \ref{fig:thinwall}). 

\begin{figure}[h]
$$\includegraphics[width=5cm]{thinwall.pdf} $$   
\begin{center}
\caption{\emph{ The idealized  state generating a null singularity by the collision of a thin-walled bubble with dS$_{d+1}$ worldvolume. Notice that WdW patches anchored at the horizon do not touch the singularity. }\label{fig:tw}}
\label{fig:thinwall}
\end{center}
\end{figure} 

The formal analysis is very similar to that of the topological crunch with the difference that the shrinking ${\bf S}^1$ is not present now. The bulk metric can be obtained therefore simply removing the $\text{d} \phi^2$ factor in \eqref{topmetric} 
\begin{equation}
\label{thinmetric}
\text{d}s^2 =  \sec ^2(u-v) \left[ -4 \, \text{d}u \text{d}v + \sin ^2(u-v) \, \text{d}\Omega^2_{d} \right],
\end{equation}
and the calculations follow very easily from the previous ones. In effect, the bulk contribution is obtained as

\begin{eqnarray}
I_{\text{bulk}}[\CW_u] &=&  -\dfrac{(d+1)V_\Omega}{8 \pi G} \int\limits^{u}_{0} \text{d}u' \int\limits^{u'}_{0} \text{d}v \; \dfrac{\tan^d(u'-v)}{\cos^3(u'-v)} \approx \dfrac{V_\Omega}{8 \pi G d} \left( \dfrac{1}{u_*-u} \right)^{d}.
\end{eqnarray}
where as usual we have performed an expansion around $u \sim u_*$ in the last equality. As the timelike surface at $u=v$ has vanishing induced metric, all codimension-one boundaries of this WdW patch vanish when the parametrization is taken to be affine along the null ones $N_{\pm}$. We need however to compute the countertems for the later. For both boundaries we get the quantitites \footnote{We omit here the normalization constants $\alpha_\pm$ as its cancellation is analogous to the previous case}
\begin{eqnarray}
\lambda_\pm &=&  \tan (u-v)\,, \\
\sqrt{\gamma}_{\pm} &=& (\lambda_\pm)^{d}\,, \\
\Theta_\pm &=& \dfrac{d-1}{\lambda_\pm}\,.
\end{eqnarray}
And the counterterms are very similar to \eqref{counterU}
\begin{eqnarray}
\label{TWct}
I^-_{\Theta} = I^+_{\Theta} &=& \dfrac{V_\Omega}{8 \pi G} \int\limits_0^{\tan u}  \text{d}\lambda \,  \lambda^{d-1} d \, \log \left(\LL\, \dfrac{d}{\lambda} \right) \\  
&=&\dfrac{ V_\Omega}{8 \pi d G} \tan^{d}u \, (d \, \log (d \, \LL \cot u)+1), \\
 &\approx& \dfrac{S}{2\pi d} \left(1+\log \left( \dfrac{V_\Omega}{4G}\right)+ d\log \left( d \,\LL\right) -\log S \right) ,
\end{eqnarray}
where we substituted again the entropy along the horizon, which remains identical as in the previous example \eqref{entropytop}. The joint contribution will also have the same form as in the previous example, therefore cancelling again the $S \log S$ leading divergence in $I_{\Theta}^{\pm}$ for the asymptotic limit $u\sim u_*$. Adding up all pieces of the action we may obtain the total complexity
\begin{eqnarray}
\CC^*\approx  a \,S \,,
\end{eqnarray}
with
\begin{eqnarray}
a= \dfrac{1}{\pi d} \left[-1+\dfrac{1}{2}d\log(2)  + d\log \left( d \,\LL \right)\right],
\end{eqnarray}
an expression that tells us again that the leading divergence is guaranteed to be positive as long as the counterterm scale satisfies $\LL \gtrsim 1$.

\begin{figure}[h]
$$\includegraphics[width=4cm]{FLRW.pdf} $$   
\begin{center}
\caption{\emph{ Maximally extended FLRW solution embedded in AdS space. The early-times approximation $a(\tilde{t}\,)\approx \tilde{t}$ guarantees that the geometry in the vecinity of $N_-$ (shaded region) is the same as in the pure AdS solutions, implying that $I^-_\Theta$ and $I_{\mathcal{V}_u}$ are identical to those of the vacuum cases. As the same is true for the near-horizon piece of $I^+_\Theta$ (in blue), the logarithmic divergence is generically cancelled provided no new dominating contributions arise from the deep interior piece of $I^+_\Theta$.}}
\label{fig:thickwall}
\end{center}
\end{figure} 


As both the latter examples come from spacetimes that are locally AdS, one might be suspicious about the seemingly miraculous cancellation of the logarithmic divergence. Nonetheless, there are reasons to think that such cancellation is generic for more realistic solutions involving a backreacting scalar field that drives a homogeneous cosmology behind the horizon. Indeed, for any negatively curved FLRW solution to enjoy a smooth horizon, the behavior of the scale factor around the time origin must be of the form $a(\tilde{t}\,) \approx \tilde{t}$. This scaling coincides with the structure present in the near-horizon region from the previous examples and therefore will yield the very same contributions for the $I_\Theta^-$ and $I_{\CV_u}$ terms. The future null counterterm $I^+_\Theta$ on the other hand, will pick up information from the full cosmological solution which in turn will depend on the details of the particular model. In the two analytic examples above, however, it is easy to see that the integrals \eqref{counterV} and \eqref{TWct} are strongly dominated by the near-horizon region, the one responsible of the logarithmic divergence. The far interior, on the other hand, contributes at most linearly to the complexity. As the cosmological solution must be that of the thin wall approximation for a neighborhood around the horizon, the logarithmic contribution from $I^+_\Theta$ will remain identical and accordingly will produce the generic cancellation of the leading divergence (cf. Figure \ref{fig:thickwall}). This of course does not prevent a possible restoration of higher than linear divergencies in both the bulk and  $I^+_\Theta$ contributions when the full cosmological dynamics is taken into account. The estimation of such effects is beyond the scope of this work. 



















\subsection{A vacuum terminal with vanishing entropy}

In this section we consider an example in which the entropy of the singularity, as defined by the volume of codimension-two sets ${\cal V}_u$, has precisely the opposite behavior to the expanding bubble models,  namely it vanishes at the singular locus. Consider the  Kasner metric in $d+2$ dimensions 
\begin{equation}
\label{kasner}
\dd s^2 = -\dd t^2 + \sum_{j=1}^{d+1} (H\,t)^{2p_j} \dd x_j^2\;,
\end{equation}
which conforms the standard vacuum solution with zero cosmological constant and $\mathbb{R}^{d}$ symmetry. Here, $H$ is an inverse-length setting a characteristic value for the expansion away from  the terminal set. Rather than a merely formal solution, the Kasner metric provides a local approximation for `small portions' ($H\Delta x_j \ll 1$) of more general singularities (cf. \cite{BKL, BKL2,BKL3,libro}), making it an object of special interest in the study of terminal spacetimes. Einstein equations impose the coefficients $p_i$ to be restricted to satisfy $\sum_i p_i = \sum_i p_i^2 =1$, where at least one of the exponents $p_i$ must be negative, indicating that at least one direction stretches as one approaches the singularity. The volume of codimension-two surfaces sitting at some constant value of $t$  always vanishes as $|t|$ in the  $t\rightarrow 0$ limit. 

In order to adapt the discussion to the symmetries of the Kasner metric, we  pick one spatial coordinate, say $x_1$, and define the singular set to be a `slab' ${\cal S}^* = \left[-{u_* \over 2} , {u_*\over 2} \right] \times {\bf R}^{d-1}$ for some finite $u_*$ measuring the $x_1$ coordinate length of the finite interval. The set of WdW patches indicated in Figure \ref{fig:kasner} intersect ${\cal S}^*$ along the nested  `slabs' ${\cal S}^*_u =   \left[-{u \over 2} , {u\over 2} \right] \times {\bf R}^{d-1}$. 

In this construction, we regard the holographic data as specified on ${\cal V}_u = \{-{u\over 2}\} \times {\bf R}^{d-1} \cup  \{{u\over 2}\} \times {\bf R}^{d-1}$, and the $x_1$ coordinate takes the role of `holographic' emergent direction. The fact that the holographic data lies on disconnected spaces, interpolated by the `bulk' WdW patches, makes this construction similar to the standard eternal AdS black hole and its dual product CFTs \cite{Maldacenaeternal}, with the crucial difference that here the entropy density 
\begin{equation}
{\tilde S} = {1\over V_{{\bf R}^{d-1}}} {{\rm Vol} ({\cal V}_u )\over 4G} \, ,
\end{equation}
vanishes as  the singularity is approached in the limit $u\rightarrow u_*$. 



Let us pick spacetime units so that the `Hubble rate' $H=1$, and pass to conformal coordinates 
\begin{equation}
\label{kasnermetric}
\text{d}s^2 = \left((1-p_1) \tau \right)^{\frac{2p_1}{1-p_1}} \left(-\text{d}\tau^2 + \text{d}x_1^2 +  \sum\limits_{i=2}^{d+1}\left((1-p_1)\tau\right)^{\frac{2(p_i-p_1)}{1-p_1}} \text{d}x_i^2 \right),
\end{equation} 
where $\tau$ is the conformal time in the $(t, x_1)$ plane. As in this case we are dealing with a Ricci flat solution, the bulk contribution of $\CW_u$ will be trivially zero. It will suffice thus to compute the expansion counterterms, joints and the YGH contribution from the singular locus. For the latter, it is easy to see from \eqref{kasnermetric} that $\sqrt{\gamma}\,K=1$, implying the very simple contribution
\begin{equation}
I_{\text{YGH}}= \dfrac{V_{{\bf R}^{d-1}}}{4\pi G}\, u \,,
\end{equation}
where $V_{{\bf R}^{d-1}}$ is the volume of the non-compact directions, appearing here in the sense that we may define a finite complexity density $\widetilde{\CC}=\CC /V_{{\bf R}^{d-1}}$. In order to compute the counterterms, we may define as usual the null coordinates by $\tau, x_1 = \frac{1}{2} (u\pm v)$. Starting with the past boundary $N_- = (u,v_0,\vec x_{i,0}),$ we find that its surface gravity is given by

\begin{figure}[h]
$$\includegraphics[width=9cm]{kasner.pdf} $$   
\begin{center}
\caption{\emph{ WdW patch for a Kasner slab ${\cal S}^*_u = \left[-{u \over 2} , {u\over 2} \right] \times {\bf R}^{d-1}$. }}
\label{fig:kasner}
\end{center}
\end{figure} 

\begin{equation}
\kappa = -\frac{2 p_1}{(p_1-1) (u+v_0)}\, ,
\end{equation}
and following the standard procedure we get the correct affine parameter
\begin{equation}
\lambda_-(u) =  \dfrac{1}{\alpha_-}(u+v_0)^{1/\delta}\, ,
\end{equation}
where we defined for simplicity $\delta= \frac{1-p_1}{1+p_1}$. We can calculate now the induced volume element and the expansion
\begin{eqnarray}
\sqrt{\gamma} &=& -\dfrac{\delta}{1+\delta}(\alpha_- \lambda_-)^\delta\,, \\
\Theta &=& \dfrac{\delta}{\lambda_-}\,.
\end{eqnarray}
Feeding it into the couterterm action we get
\begin{eqnarray}
I_{\Theta}^- &=& \dfrac{ V_{{\bf R}^{d-1}}}{8 \pi G} \int\limits_{\lambda_-(u_0)}^{\lambda_-(u)} \text{d} \lambda_- \, \dfrac{\delta^{2}}{\delta+1} \,\alpha_-^\delta \, \lambda^{\delta-1} \, \log\left(\dfrac{\LL \,\delta}{\lambda_-} \right) \\  
&=& -\dfrac{ V_{{\bf R}^{d-1}}}{8 \pi G} \dfrac{1}{\delta+1}(u+v_0)\left[   1+ \delta \log \left(\delta \, \LL \alpha_- \right) -\log \left(u+v_0 \right)  \right]  - (u \leftrightarrow u_0) .\nonumber
\end{eqnarray}

Repeating the procedure above for the future null boundary $N_+$ we can see that the counterterm contribution is given by an almost identical expression where we must exchange the roles $u, u_0 \leftrightarrow u$ and $v_{0} \leftrightarrow v_{0}, v_*$ with $v_*=-v_0=-u_0=u_*$ the value at the singularity.
\begin{eqnarray}
I_{\Theta}^+ &=& -\dfrac{ V_{{\bf R}^{d-1}}}{8 \pi G} \int\limits^{\lambda_+(v_*)}_{\lambda_+(v_0)} \text{d} \lambda_+ \, \dfrac{\delta^{}}{\delta+1} \,\alpha_+^\delta \, \lambda_+^{\delta-1} \, \log\left(\dfrac{\LL \,\delta}{\lambda_+} \right) \\  
&=& -\dfrac{ V_{{\bf R}^{d-1}}}{8 \pi G} \dfrac{1}{\delta+1}(u+v_0) \left[  1+ \delta\,\log \left( \delta \LL \alpha_+  \right) -\log \left(u+v_0 \right) \right] .\nonumber
\end{eqnarray}
Now, we must calculate the contribution from the joints of these surfaces. Choosing the normal vectors
\begin{eqnarray}
k_+ &=& \alpha_+ (d\tau+dx_1)\,,\\
k_- &=& \alpha_- (d\tau-dx_1)\,,
\end{eqnarray}
we get the contribution
\begin{equation}
I_{\CV_u}= \dfrac{ V_{{\bf R}^{d-1}}}{4 \pi G} \dfrac{\delta}{\delta+1}\left(u+v_0\right) \log \left( \alpha_+ \, \alpha_- \,\left((u+v_0)\dfrac{\delta}{\delta+1} \right)^{\frac{\delta-1}{\delta}} \right)\,,
\end{equation}
and similarly for the south tip
\begin{equation}
I_{\southcorner}= -\dfrac{ V_{{\bf R}^{d-1}}}{8 \pi G} \dfrac{\delta}{\delta+1}\left(u_0+v_0\right) \log \left( \alpha_+ \, \alpha_- \,\left((u_0+v_0)\dfrac{\delta}{\delta+1} \right)^{\frac{\delta-1}{\delta}} \right)\,,
\end{equation}
and as we see, the dependence on $\alpha_{\pm}$ will cancel with that of the counterterms above. The entropy along the horizon in this case will be

\begin{equation}
S= -\dfrac{2\delta}{\delta+1} \dfrac{V_{{\bf R}^{d-1}}}{4G}(u+v_0)\, ,
\end{equation}
so we may rewrite again everything as a function of the entropy
\begin{eqnarray}
\label{kasnerYGH}
I_{\text{YGH}} &=& \dfrac{\delta+1}{2\pi \delta} (S_0/2-S)\, ,\\
2(I_{\Theta}^+ +I_{\Theta}^-)&=&\dfrac{S}{\pi \delta} \left[ 1+\log\left( \frac{\delta}{\delta+1}\, \frac{V_{{\bf R}^{d-1}}}{2G}\right) +\delta \log( \delta \,\LL )-\log S \right] - \dfrac{1}{2} \left( S \leftrightarrow S_0 \right)\, , \\
I_{\CV_u} &=& \dfrac{S}{\pi\delta} \dfrac{\delta-1}{2}\left[ \log\left(\dfrac{V_{{\bf R}^{d-1}}}{2G}\right) -\log S\right]\, ,\\
I_{\southcorner} &=& \dfrac{S_0}{ \pi\delta} \dfrac{\delta-1}{4}\left[ -\log\left(\dfrac{V_{{\bf R}^{d-1}}}{2G}\right) +\log S_0\right]\,,\label{kasnertip}
\end{eqnarray}
where $S_0$ is a constant that stands for the entropy evaluated at the south tip of the WdW patch $(u_0, v_0$). As we see, we recover the same structure for the counterterm as in the expanding case \eqref{TWct} and the black hole (cf. \cite{Myerstdep}) but in which the constant $\delta$ seems to play now the role of the codimension-2. Interestingly such effective dimension can in fact recover the value $\delta = d$ by considering the `holographic coordinate' $x_1$ to be the ripping direction in the most isotropic case, i.e. $p_1 = \frac{1-d}{d+1}$ and $p_{i \neq 1}=\frac{2}{d+1} $. Such values for the Kasner exponents correspond furthermore to the near-singularity approximation of the Schwarzschild black hole metric.


From equations \eqref{kasnerYGH} to \eqref{kasnertip}, we see that we obtain a log-linear locking for the total complexity density in the Kasner solution. Particularly, we can extract a growth rate of the form
\begin{eqnarray}
\delta \widetilde{\CC}^* &=&  \left( a\, + b\log \tilde{S} \right) \delta \tilde{S}\, ,
\end{eqnarray}
with
\begin{eqnarray}
a &=&\dfrac{1}{\pi \delta} \left[ -\delta + \dfrac{\delta+1}{2} \log \left(\dfrac{1}{2G}\right) +\log\left( \dfrac{\delta}{\delta+1} \right)+ \delta\log(\delta \, \LL )  \right]\, ,\\
b &=& -\dfrac{\delta+1}{2 \pi \delta}\,  ,
\end{eqnarray}
where we have restored the  entropy density $\tilde{S}=S/V_{{\bf R}^{d-1}}$. As we can see, the terminal behavior of the complexity is now controlled by the balance of the linear and logarithmic pieces, in turn depending on the UV/IR character of the scale $\LL$. Within the validity of the Kasner approximation, however, we are forced to consider entropies that do not exceed the size of the effective Kasner patch, i.e. $S \ll G^{-1}$, implying that the term in $\sim \log G$ becomes always dominant at late times. Since $\delta$ is a strictly possitive quantity, this linear dominance cannot be contrarested by any choice of $\LL$ as doing so would require to pick transplanckian values of the counterterm, taking us out of the realm of the effective theory action. Accordingly, we obtain the generic late time behaviour
\begin{equation}
\delta \widetilde{\CC}^* \approx a\,  \delta \tilde{S}\, .
\end{equation}
where $a$ is a positive quantity by the considerations above. For the case of the Kasner singularity, we therefore see that complexity is a decreasing quantity, an effect that signals the dominance of the strong shriking of the effective Hilbert space over the natural tendency of complexity to grow in sistems at equililibrium. 

\newpage
\section{The local component of terminal complexity}
\label{sec:local}

\noindent

As emphasized in the introduction, a remarkable property of the AC complexity prescription is the occurrence of a quantitatively important  contribution coming directly from the singularity through the evaluation of the YGH term. Despite the fact that its validity is tied to that of the effective theory description in a strong gravity regime, this contribution is argued to be of vital importance when computing the AC complexity, and seems to be the only object that is known so far in the holographic dictionary providing an order one contribution to a finite quantity which is calculated in the vecinity of a singularity.

The YGH contribution is local and formally extensive over the singular set ${\cal S}^*$. However, the volume form is not generally defined at ${\cal S}^*$, which makes the notion of `extensivity' non-trivial.  In order to elucidate this point, let us parametrize the near-terminal metric by  a Gaussian normal  coordinate $\tau$. This foliates  the near-terminal  spacetime into spacelike surfaces $\Sigma_\tau$, according to the proper-time distance to $\CS^*$. In defining a metric on the $\Sigma_\tau$ slices, we extract a conventional power of the proper time according to the ansatz
\begin{equation}\label{locs}
\dd s^2 = -\dd{\tau}^2 + (\tau H)^{2\gamma/d} \, \dd\Sigma_\tau^{\;2}\;,
\end{equation}
where $H^{-1}$ sets the characteristic scale for the expansion away from  the terminal set. In general,  the $d$-dimensional  metric  $\dd\Sigma_\tau^2$  does not have a smooth limit  as $\tau \rightarrow 0^+$, but we may choose the conventional exponent $\gamma$
in such a way that its volume form   does have a smooth limit. We shall actually assume that this volume form  is analytic in $\tau$, since this will be a property of all examples we study (it would be interesting to assess the generality of this assumption.) We will refer to such notion of volume for ${\CS}^*$ as the `comoving volume' of the terminal set and 
denote its measure as $\dd {\rm Vol}_c $. 


In this notation, the YGH term in the action is  computed as
\begin{equation}\label{ygh}
\tilde{I}[{\CS}^*]_{\rm YGH}= {1\over 8\pi G} \lim_{{\tau}\rightarrow 0^+} \partial_{\tau} \big[(H{\tau})^{\gamma} \,{\rm Vol}_c [\Sigma_\tau]\big]\;.
\end{equation}
 Picking the term proportional to the comoving volume ${\rm Vol}_c [{\cal S}^*]$ of the singular set,  we find that the YGH term vanishes for $\gamma >1$ and is infinite for $\gamma <1$, except perhaps the case $\gamma =0$ where the answer depends on the possible occurrence of logarithmic terms in the terminal expansion near $\tau=0$. The most interesting case is $\gamma =1$, for which one defines a nontrivial  `comoving complexity density' at the singular set, given by $H/8\pi G$. 
 
 The black hole singularity has $\gamma =1$ and thus presents a purely local contribution to complexity. In fact, this feature appears to be quite general. At spherically symmetric black-hole singularities we have a vanishing ${\bf S}^{d-1}$ and an expanding `radial' direction. Hence, the metric is locally of the Kasner form, i.e. 
 \begin{equation}\label{km}
 \dd s^2 = -\dd \tau^2 + \sum_{j=1}^{d} (H\tau)^{2p_j } \, \dd \sigma_j^2\;,
 \end{equation}
 with a particular choice of Kasner parameters $p_c = \frac{2}{{d}}$ for  $d-1$ `crunching' directions and $p_r = -1+2/d$ for the `ripping' direction. More generally, the Kasner parameters are restricted to satisfy 
 the sum rules $\sum_j p_j  = \sum_j p_j^2 =1$ and any such metric can be put in the form (\ref{locs}) with $\gamma =1$, with
 `comoving' metric
  \begin{equation}\label{comov}
 \dd \Sigma_\tau^2 = \sum_j (\tau H)^{2p_j  - 2/d} \,\dd \sigma_j^2
 \;.
 \end{equation}
  In particular, it has a smooth comoving volume form,  
 \begin{equation}
 \dd{\rm Vol}_c [ \Sigma_\tau] = \wedge_{j=1}^d \dd \sigma_j
 \end{equation}
  as a simple consequence of the sum rule $\sum_j p_j =1$.    
 


   The $\gamma=1$ property and the resulting non-vanishing `complexity density' persist if we let the Kasner parameters depend smoothly  on the `longitudinal' $\sigma_j$. In fact, the  classic results of ref. \cite{BKL,BKL2,BKL3} (BKL) indicate that such a `generalized Kasner'  metrics 
 furnish a good local approximation of the near-singular region (after a slight generalization involving local rescalings and frame rotations.) 
 
 
 
 \subsection{Local terminal complexity and coarse-graining}

\noindent

The remarkable properties of the local YGH contribution  beg the question of whether we may be able to isolate this term in more physical terms. A natural strategy in this case is to focus on the extensivity of the local contribution, a property not shared by the full AC complexity. As the evaluation of the null boundary contributions generally requires a complete knowledge of the metric, we take in this section a more conservative point of view, and study the pieces of AC complexity that are purely geometrical, i.e. that do not depend on formal `gauge' choices of parametrization or the addition of extra counterterms. We define thus this `geometric complexity' and denote it as $\CC_g$ as the Einstein-Hilbert and YGH contributions to the action on $D^-(\CS^*)$
\begin{equation}\label{ac}
\CC_g^*(u)= \tilde{I}[D^-(\CS^*)]_{\rm bulk} + \tilde{I}[{\cal S}^*]_{\rm YGH}\;.
\end{equation}
In order to illustrate the point on the extensivity of this quantity, we can do so by focusing on the simpler case of vacuum solutions. A vacuum solution is a $(d+1)$-dimensional Einstein manifold whose metric satisfies
\begin{equation}\label{eme}
R_{\mu\nu} = {2\Lambda \over d-1} g_{\mu\nu}\;,
\end{equation}
with cosmological constant $\Lambda$ and no matter degrees of freedom. The bulk contribution to the on-shell action is then
proportional to the spacetime volume
 \begin{equation}\label{bulkc}
 I[X]_{\rm bulk} = {1\over 16\pi G} \int_X (R-2\Lambda) = {\Lambda \over 4\pi G (d-1)} \,{\rm Vol} [X]\;.
 \end{equation}
Assuming a $\gamma=1$ singular set ${\cal S}^*$  with non-vanishing complexity density, we have a full geometric complexity given formally by
\begin{equation}\label{fullq}
\CC_g[{\cal S}^*] =  {\Lambda \over 4\pi G (d-1)} {\rm Vol}\left[D^- ({\cal S}^*)\right] + {H \over 8\pi G} {\rm Vol}_c [{\cal S}^*] \;.
\end{equation}
While the YGH term is extensive along the comoving volume of ${\cal S}^*$, the bulk contribution is extensive in the full spacetime volume of the past domain of dependence. Considering the case $\Lambda <0$, as corresponds to states in an AdS/CFT context, we have a negative-definite bulk contribution, leading to a `subextensivity' property of the full quasilocal complexity. Indeed, under a
coarse-graining of the singular set ${\cal S}^* = \cup_i {\cal S}^*_i$ as indicated in Figure \ref{fig:subextensive}, the expression (\ref{fullq}) satisfies 
\begin{equation}\label{sube}
\CC_g[{\cal S}^*] = \CC_g \left[\cup_i {\cal S}^*_i \right] \leq \sum_i \CC_g[{\cal S}^*_i]\;.
\end{equation}
The inequality is reversed (corresponding to superextensivity) for vacuum singularities in $\Lambda >0$ spaces. The deviation from
extensivity  would disappear if the bulk contributions were to become negligible, a situation we may expect in the limit of extreme coarse graining, illustrated in Figure \ref{fig:ultralocal}. 

\begin{figure}[t]
$$\includegraphics[width=8cm]{subextensive.pdf} $$   
\begin{center}
\caption{\emph{ When the bulk action is dominated by a negative cosmological constant, the bulk contribution to the AC terminal complexity of  $\CS^*$ is subextensive. While the YGH contribution is extensive over $\CS^*$, the bulk contribution is more negative for the larger set (yellow) than it is for
the union of the smaller sets (brown).  }\label{fig:subextensive}}
 \end{center}
\end{figure} 

In this case, the limit of infinite coarse-graining does isolate the YGH term. To be more precise, we require that the bulk contributions be consistently smaller than the YGH contribution for small subsets of ${\cal S}^*$. We can check this explicitly for $\gamma =1$ vacuum singularities  described by (\ref{fullq}) and admitting a local Kasner description. Let us consider a fine partition of the singular set by subsets ${\cal S}^*_\epsilon$ with comoving volume of order $\epsilon^d$. The condition for the bulk contribution to be negligible for small sets is that
\begin{equation}\label{epd}
{{\rm Vol}\left[D^- ({\cal S}^*_\epsilon)\right] \over {\rm Vol}_c \left[{\cal S}^*_\epsilon\right]} \sim \epsilon^{\,a}
\;,\end{equation}
with $a >0$. 
Instead of computing the volume of the past domain of dependence, $ D^- ({\cal S}^*_\epsilon)$,  it is easier to compute the volume of the larger set $B^- ({\cal S}^*_\epsilon)$, which `boxes' it
in the standard coordinate frame. If $\tau_\epsilon$ is the maximal value of the $\tau$ coordinate in $D^- ({\cal S}^*_\epsilon)$, the
$\epsilon$-box is defined by the full $\tau\leq \tau_\epsilon$ subset with given comoving coordinates covering ${\cal S}^*$, c.f. Figure (\ref{fig:box}). 
Evidently, ${\rm Vol}\left[B^-({\cal S}^*_\epsilon)\right] \geq {\rm Vol}\left[D^- ({\cal S}^*_\epsilon)\right]$, so that it is enough to establish the condition (\ref{epd}) for $B^- ({\cal S}^*_\epsilon)$.


\begin{figure}[t]
$$\includegraphics[width=8cm]{ultralocal.pdf} $$   
\begin{center}
\caption{\emph{ When the bulk volume remains sufficiently bounded in the vicinity of the terminal surface, the local complexity of ${\CS}^*$ results from the limit of an extreme coarse graining.  }\label{fig:ultralocal}}
 \end{center}
\end{figure} 






In order to construct explicitly $B^- ({\cal S}^*_\epsilon)$  for the Kasner metric (\ref{km}) we define ${\cal S}^*_\epsilon$ to be a  $d$-dimensional cube  in the $\sigma$ coordinates with common extent $\Delta \sigma_j = \epsilon$. Its comoving volume is ${\rm Vol}_c \left[{\cal S}^*_\epsilon\right] = \epsilon^d$ and the past domain of dependence, $D^- ({\cal S}^*_\epsilon)$, is a trapezoid with base ${\cal S}^*_\epsilon$ and a  ridge with the topology of a $(d-1)$-dimensional cube, determined by the intersection of light rays in the spacetime plane with faster past-convergence. For any direction $\sigma_j$ we can define a corresponding conformal time coordinate $\eta_j$ such that light rays propagate with unit slope in the $(\eta_j, \sigma_j)$ plane. The explicit relation between $\eta_j$ and the proper time is
\begin{equation}
(1-p_j) H \eta_j = (H\tau)^{1-p_j}
\;,
\end{equation}
where $p_j$ is the Kasner exponent in the direction $\sigma_j$. Light rays whose $\sigma_j$ separation is $\epsilon$ at  $\tau=0$ converge in the past at $\tau_\epsilon^{(j)}$ given by
\begin{equation}
H\tau_\epsilon^{(j)} = \left((1-p_j) {H\epsilon \over 2}\right)^{1\over 1-p_j}\;.
\end{equation}
  Thus, the past domain of dependence of the full ${\cal S}^*_\epsilon$ set is determined by the smallest $\tau_\epsilon^{(j)}$ or, equivalently, by the {\it largest} Kasner exponent which we denote by $p_c$:
\begin{equation}\label{taue}
H\tau_\epsilon = \left((1-p_c){H\epsilon \over 2}\right)^{1 \over 1-p_c}\;.
\end{equation}
 With these ingredients we can compute the volume
  of the $\epsilon$-box as
  \begin{equation}\label{vole}
  {\rm Vol}\left[B^- ({\cal S}^*_\epsilon)\right] = \int_0^{\tau_\epsilon} d\tau \,(H\tau) \, \epsilon^d = {1\over 2H} \,(\tau_\epsilon H)^2 \,\epsilon^d\;,
  \end{equation}
  and verify (\ref{epd}) with $a = 2(1-p_c)^{-1}$. 
  
\begin{figure}[t]
$$\includegraphics[width=8cm]{box.eps} $$   
\begin{center}
\caption{\emph{ Comparison between the $\epsilon$-box and the past domain of dependence of ${\cal S}^*_\epsilon$. }\label{fig:box}}
 \end{center}
\end{figure} 


For   solutions with matter degrees of freedom we need to check that the Lagrangian ${\cal L}_m$ is not too singular. For instance, we may study the  FRW terminal with metric 
\begin{equation}\label{frw}
ds^2 = -d\tau^2 + a(\tau)^2 \,d\Sigma^2\;
\end{equation}

which presents a singularity at $\tau=0$. By construction, the non-singular comoving volume is just given by the volume of the homogeneous and isotropic surfaces $\Sigma$, so that the complexity exponent  $\gamma$ can be read off from the short-time asymptotics of the scale factor $a(\tau)$. Since FRW metrics require non-trivial matter degrees of freedom, we follow standard practice and model them as a perfect fluid with squared speed of sound equal to $w = p/\rho$, where $p$ denotes the pressure and $\rho$ the energy density. Then, we have the standard solution $\rho \;a^{d(1+w)} = $ constant, which leads to 
$a(\tau) \sim \tau^{2 /d(1+w)}$ or, equivalently 
\begin{equation}
\gamma_{\rm FRW} = {2 \over 1+w}\;.
\end{equation}

Approximating the action dimensionally as the volume integral of the energy density $\rho \sim \tau^{-2}$, we estimate
\begin{equation}\label{aces}
I\left[B^- ({\cal S}^*_\epsilon)\right]_{\rm bulk} \propto \epsilon^{\,d} \int_0^{\tau_\epsilon} d\tau \,\tau^\gamma {1\over \tau^2} \sim \epsilon^d \,\tau_\epsilon^{\gamma-1}\;.
\end{equation}


\begin{table}
\label{tablaFLRW}
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
  & \cellcolor{gray!25} AdS & \cellcolor{gray!25} Milne &\cellcolor{gray!25} Matter & \cellcolor{gray!25}Radiation & \cellcolor{gray!25}Stiff matter\\
\hline
 \cellcolor{gray!25} $\omega$ &  $-1$ & $2/d -1$ & $0$ & $1/d$ &		$1$ \\
\hline
\cellcolor{gray!25} $\gamma$ &  $\infty$ & $d$ & $2$ 		& $2d/(d+1)$ & $1$		 \\
\hline
\cellcolor{gray!25} $a(\tau)$ & $\sim e^{H\tau}$ &  $\sim \tau $ &  $\sim \tau^{2/d}$  & $\sim \tau^{2/(d+1)}$ & 	$\sim \tau^{1/d}$	\\
\hline
\end{tabular}
\end{center}
\caption{\textit{Scalings for different cosmological solutions as classified by the equation of state of a perfect fluid.} }
\end{table}

The condition for the coarse-graining procedure to be well-defined is now
\begin{equation}\label{genco}
{I\left[B^- ({\cal S}^*_\epsilon)\right]_{\rm bulk} \over {\rm Vol}_c [{\cal S}^*_\epsilon]} \sim \epsilon^{\,a}\;, \;\;\;a>0\;.
\end{equation}
The physical condition that  the matter equation of state remains  strictly below the stiff limit, $w<1$, implies that $\gamma >1$ and thus (\ref{genco}) is satisfied 
 provided $\tau_\epsilon$ scales with a positive power of $\epsilon$. This
happens for any solution which {\it decelerates} away from the singularity, since the FRW conformal time is given by 
\begin{equation}\label{frwco}
H\eta = \dfrac{d}{d-\gamma}\left(H \tau\right)^{d-\gamma \over d}\;.
\end{equation}
It is precisely for decelerating singularities that we have $\gamma < d$ and $\tau_\epsilon \sim \epsilon^{d\over d-\gamma}$
scaling with a positive power of $\epsilon$, leading to an automatically well-defined coarse-graining limit.

The situation is less clear for FRW metrics that {\it accelerate} away from the singularity, corresponding to $\gamma \geq d$. Now the FRW conformal time plummets to $-\infty$ as $\tau\rightarrow 0^+$. The problem in this case is that $D^- ({\cal S}^*_\epsilon)$ is not itself well defined, as any past light cone emanating from $\tau =0$ and converging at a finite value $\tau_0$ subtends an infinite comoving volume at the terminal surface. To address this point we regularize the terminal surface by bringing it slightly before the singularity at $\tau =\delta$, as indicated in Figure (\ref{fig:frwacc}).  In other words, we compute the past domain of dependence for a small, $\epsilon$-sized subset of $\Sigma_\delta$ rather than ${\cal S}^*$. Let us denote this set ${\cal S}^\delta_\epsilon$. Its past  domain of dependence, $D^- ({\cal S}^\delta_\epsilon)$, has an earliest proper time which is a function of both $\epsilon$ and $\delta$, 
\begin{equation}
\tau_0 (\epsilon,\delta)  = {1\over H} \left((H\delta)^{d-\gamma \over d} + {d-\gamma \over d} {H\epsilon \over 2}\right)^{d \over d-\gamma}\;.
\end{equation}
For $\gamma >d$, this quantity  vanishes linearly in $\delta$ as the terminal time cutoff is removed  at fixed $\epsilon$. 
Hence, when we repeat the estimate 
(\ref{aces}) we find that 
\begin{equation}\label{newaces}
I\left[B^-({\cal S}^\delta_\epsilon)\right]_{\rm bulk} \propto \epsilon^{\,d} \int_{\delta}^{\tau_0} d\tau\, \tau^\gamma \,{1\over \tau^2} \sim \epsilon^d (\tau_0^{\,\gamma -1} - \delta^{\,\gamma-1}) \longrightarrow 0\;,
\end{equation}
as $\delta \rightarrow 0$ at fixed $\epsilon$, since both terms vanish in the limit. Therefore, the bulk contribution vanishes when we remove the regularization at fixed comoving volume, even before we take $\epsilon \rightarrow 0$. 


\begin{figure}[t]
$$\includegraphics[width=9cm]{frwacc.eps} $$   
\begin{center}
\caption{\emph{The regularized terminal ${\cal S}^\delta_\epsilon$ and its past domain of dependence.  }\label{fig:frwacc}}
 \end{center}
\end{figure} 



As we have seen thus, the YGH piece of the action can be isolated as a local contribution to the complexity under an extreme coarse-graining procedure. In this respect, the relation of the YGH term  to the full quasilocal  complexity  is analogous to the relation between the  classical thermodynamic entropy, obtained through coarse-graining, and the exact von Neumann entropy of a quantum many-body state.




 
\subsection{Terminal complexity and the arrow of time}

\noindent

If we regard the generalized Kasner behavior as `generic' we may be tempted to say that all spacelike singularities tend to have a non-vanishing  local complexity density. On the other hand, there are important examples of singularities whose YGH contribution vanishes, as is the case of those  occurring in standard FRW spacetimes. 

To bring this simple point home, we can apply \eqref{ygh} to the standard FRW metric
\begin{equation}
ds^2 = -d\tau^2 + a(\tau)^2 \,d\Sigma^2\;,
\end{equation}
with a singularity at $\tau=0$. As mentioned in the previous section, standard solutions to the Einstein equations for a perfect fluid with equation of state $p=\omega \rho$ yield terminal metrics of the form \eqref{locs} with  $\gamma = {2 \over 1+w}$. This result implies that the only FRW singularity with a finite complexity density is the slightly unphysical case with `stiff matter', $w=1$, leading to $\gamma=1$. On the other hand, a formally infinite contribution to the complexity density, associated to $\gamma <1$, would require $w>1$  in the FRW context, i.e. a violation of  the energy conditions on the matter degrees of freedom. 

Imposing the physical condition that the matter is strictly below the `stiff' limit, $w<1$, we have $\gamma >1$, implying  a {\it vanishing} local complexity. Hence, we find that  `ordered' singularities of FLRW type have a vanishing local contribution to holographic complexity whereas more generic (Kasner) ones do not. This feature suggests that holographic complexity might be a suitable diagnostic tool to classify GR singularities according to their nature, an effort which goes back to \cite{Penrose, misner, BKL, BKL2, BKL3 }.

In \cite{Penrose} Penrose gave a local criterion for the complexity of a singularity. The basic observation was that `ordered' singularities, like the ones in FLRW models, have vanishing Weyl curvature, whereas more generic ones, such as those arising in gravitational collapse, have a generically divergent Weyl tensor.  Penrose argued that the Weyl criterion would be associated to a large gravitational entropy flowing into the singularity, a suggestion based on the heuristic picture of a generic cosmological crunch, full of chaotic black hole collisions (see Figure \ref{fig:penrosecriterion}). Since black holes are known to carry entropy, a corresponding notion of entropy may be assigned to the union of all singularities enclosed by the colliding black holes. 


\begin{figure}[t]
\begin{center}
\includegraphics[height=6cm]{Penrosecrunchdoble2.png}
\end{center}
\caption{\emph{Schematic picture representing Penrose's argument. In the left, a perfectly homogeneous bouncing cosmology. In the right, a more realistic cosmology undergoing a crunch with scattered black holes. }}
\label{fig:penrosecriterion}
\end{figure}

As the Weyl tensor does not seem to be directly related with any known measure of entropy in the context of AdS/CFT, one basic observation of this section is that holographic complexity, rather than entropy, might provide a more natural language in the seek for a classification of singularities, a picture supported by the behavior of the YGH contribution to AC complexity in the Kasner and FLRW spacetimes.


As it turns out, however, there is an interesting twist to this story. According to the classic  BKL analysis \cite{BKL,BKL2,BKL3}, the vicinity of a generic spacelike singularity is not quite described by a single generalized Kasner metric, but rather an oscillating  regime where a series of `epochs' succeed one another, each epoch being locally described by a generalized Kasner solution of the type (\ref{km}). The values of the Kasner parameters, $p_j$, change from one epoch to the next one in a deterministic but chaotic manner \footnote{Since the proposal of the BKL hypothesis, some objections have been raised (e.g. \cite{BarrowTipler}) that question the validity of the approximation. Numerical simulations of gravitational collapse (cf. \cite{Singularitynumerics1, Singularitynumerics2} ) however have shown agreement with the BKL picture.}. In addition, the frame determining the special coordinates $\sigma_j$ in (\ref{km}) undergoes a rotation, and furthermore the induced volume form at fixed $\tau$ is rescaled by a finite factor which we may absorb in the dimensionful expansion parameter $H$. As a result, the geometry in the $n$-th epoch is well approximated by 
\begin{equation}\label{nth}
ds^2 |_{(n)} = -d\tau^2 + (H_n \tau)^{2/d} \;d^2\Sigma_\tau^{(n)}\;,
\end{equation}
where $d^2 \Sigma_\tau^{(n)}$ is a rotated version of (\ref{comov}) with Kasner parameters $p_j^{(n)}$. All epochs are described
by $\gamma=1$ metrics but, crucially, they have slightly different parameters $p_j^{(n)}$ and $H_n$.  In particular, the substitution rule for the expansion parameter follows the recurrence relation
\begin{equation}\label{eva}
H_{n+1} = (2p_r^{(n)} + 1) \,H_n\;,
\end{equation}
where $p_r^{(n)} <0$ is always the `ripping' parameter of the $n$-th epoch. Since $2p_r^{(n)} + 1 < 1$ for all $n$, the series of $H_n$ is monotonically decreasing. 

\begin{figure}[h]
$$\includegraphics[width=5cm]{BKL.jpeg} $$   
\begin{center}
\caption{\emph{ Schematic picture of a BKL singularity formed in a generic anisotropic black hole collapse. }
\label{fig:BKLsingularity}}
\end{center}
\end{figure} 



If we compute the YGH contribution to complexity by placing a regulating surface and taking the limit, the result of the complexity density is determined by the limit of $H_n$. Namely it is proportional to 
\begin{equation}\label{infp}
 \prod_{\rm epochs} (2p_r +1)\;.
 \end{equation}
 
According to the analysis of \cite{BKL,BKL2,BKL3} the truly generic singularity features an infinite number of Kasner epochs. In this situation  the  product (\ref{infp}), featuring  an infinite set of numbers in the open interval $(0,1)$,  is bound to vanish for almost all singularities as the induced volume on the successive Kasner slices becomes diluted as the singularity is approached. Ultimately, a cutoff at Planck time from the singularity must be imposed, implying that the complexity computed by this ansatz would have a finite suppression factor determined by the number of epochs taking place until Planck time. An estimation of the the number of Kasner epochs or the physical scale parameter $H$ for realistic cosmologies depends on the dynamical details of the setup \footnote{For realistic cosmologies such as the one of our universe, it has been argued that the BKL analysis undergoes only an order 1 number of Kasner epochs \cite{Henneaux}.}, limiting thus our ability to quantify generically the order of the supression factor \eqref{infp}.

\section{Conclusions and outlook}
\label{sec:conclusions}

\noindent

In this chapter we have introduced quasilocal notions of AC complexity for terminal sets such as spacelike singularities in General Relativity. The basic idea is to build WdW patches restricted to the past causal domain of the singular set. Holographic data are associated to codimension-two surfaces on corresponding horizons, assigning a notion of entropy to a singularity by looking at the area of these codimension-two sets. 

Within our `terminal complexity' definition, we have studied solutions with non-trivial entropy dynamics, showing the strong impact on complexity dynamics of a varying Hilbert space already at the level of the leading bulk approximation. In particular, we study exact solutions with divergent entropy, given by Coleman-de Luccia type solutions, and also patches of the  Kasner spacetime with vanishing entropy at the singularity, representing the local description of generic singularities in GR. We find the remarkable result that in these two very different situations, the terminal AC approaches a unified linear form in terms of the entropy
\begin{equation}
\delta \CC^*  \approx a \, \delta S  + \dots \,,
\end{equation}
up to $u$-independent constants and subleading terms.  Although the detailed form of the coefficient $a$  depends on the particular solution, some general properties are to be noticed. In particular, we find the general behavior
\begin{equation}
a = a_1 + a_2\,\log \LL\;,
\end{equation}
in appropriate units\footnote{ These are given by the AdS radius of curvature for the expanding bubble examples, and by the inverse Hubble scale $H^{-1}$ for the Kasner example.}.  Both $a_1$ and $a_2$ are strictly positive constants for all dynamical scenarios, therefore relegating negative values of $a$ only to those choices of $\LL$ that correspond to UV scales ($\LL \ll 1$) in the case of the expanding scenarios or even transplanckian ($\LL \ll \ell_{\text{Planck}}$) for the local case. Remarkably, this class of solutions comprise the most radical example of sensitivity of complexity to $\LL$ as they are the only known ones for which the late-time dynamics is qualitatively affected by the size of this scale. If one is to believe that the monotonic growth must be a generic property of terminal complexity in the expanding cases, the result above forces us to consider $\LL$ as an IR scale of the same order or lower than the the lowest scale present in the CFT, i.e. the curvature radius of the boundary metric.

In brief, we observe that an `entropic locking' of AC complexity arises when the entropy has strong dynamics near a spacelike singularity. On general grounds, we can imagine that the complexity grows linearly within a fixed Hilbert space, but it may have more complicated dynamics when the effective dimensionality of the Hilbert space, of order ${\rm exp}(S)$, changes abruptly with time. This was the situation found in \cite{rabinovc} in cases where the complexity was dominated by strong time-dependence of UV degrees of freedom. In the situations described in this paper, we are only concentrating in IR sectors, in the holographic sense, but again the effective Hilbert spaces have strongly time-dependent dimensionality and this phenomenon dominates the rate of change of complexity. 


Next, our results shed some light to the old program of classifying GR singularities according to their inherent complexity,(cf. \cite{Penrose, misner, BKL, BKL2, BKL3 }), which acquires an interesting outlook when combined with holographic ideas, providing a suitable language for these hypotheses. 

In particular we find that the  YGH term evaluated at the singularity defines a `complexity density' which serves as a holographic version of the Weyl curvature criterion by Penrose. We show that this contribution can be isolated  from the terminal AC complexity by a coarse-graining procedure, and we explicitly check that this quantity sets apart `simple' singularities, such as the one at a FRW crunch, from `complex' ones, such as the generic black hole singularity.  

 Nonetheless, within the local description of generic singularities, as presented in the classic BKL analysis, our ansatz assigns  a vanishing  complexity density to the formal infinite sequences of chaotic Kasner `epochs'. Since these chaotic structures are generic in the light of the BKL analysis, we would conclude that the  local complexity density of generic spacelike singularities is zero. We find this phenomenon puzzling, and consider that it begs the question of the proper interpretation of the scale $H$ and the order of the supression factor for realistic cosmologies within an effective GR approach.

















\newpage

